A Survey on Programmatic Weak Supervision

Labeling training data has become one of the major roadblocks to using machine learning. Among various weak supervision paradigms, programmatic weak supervision (PWS) has achieved remarkable success in easing the manual labeling bottleneck by programmatically synthesizing training labels from multiple potentially noisy supervision sources. This paper presents a comprehensive survey of recent advances in PWS. In particular, we give a brief introduction of the PWS learning paradigm, and review representative approaches for each component within PWS's learning workflow. In addition, we discuss complementary learning paradigms for tackling limited labeled data scenarios and how these related approaches can be used in conjunction with PWS. Finally, we identify several critical challenges that remain under-explored in the area to hopefully inspire future research directions in the field.

==> 03-application.tex <==
\section{Datasets and Applications}
\label{sec:dataset}

In this section, we briefly mention existing datasets and applications in PWS. 
Very recently, WRENCH~\cite{zhang2021wrench}, a comprehensive benchmark for PWS, is released along with 14 classification datasets and 8 sequence tagging datasets covering text, video, and tabular data; and WALNUT~\cite{zheng2021walnut} is another benchmark for semi-PWS with a focus on Natural Language Understanding tasks.

\paragraph{Natural Language Processing.}
In natural language processing, text classification is a popular application area for PWS~\cite{ren2020denoising,yu-etal-2021-fine,shu2020learning}.  
In addition, some works apply PWS on other field of studies, such as relation extraction~\cite{zhou2020nero,liu2017heterogeneous,Mallory2020ExtractingCR}, named entity recognition~\cite{safranchik2020weakly,lison2020named,li2021bertifying,lan2020connet,fries2017swellshark}, and dialogue systems~\cite{DBLP:conf/aaai/MallinarSUGGHLZ19}.

\paragraph{Computer Vision.}
Researchers also explore the applications of PWS on vision domain, \eg, image classification~\cite{das2020goggles}, image segmentation~\cite{hooper2020cut}, video analysis~\cite{fu2020fast,Varma2019multi}, scene graph prediction~\cite{chen2019scene}, and autonomous driving~\cite{Weng2019UtilizingWS}.

\paragraph{Biomedical.}
There are various applications of PWS on areas in biomedical domain, such as  genome study~\cite{Kuleshov2019AMD}, bioinformatics~\cite{fries2017swellshark,Mallory2020ExtractingCR}, clinical data~\cite{Fries2019WeaklySC,Fries2021OntologydrivenWS,Wang2019ACT}, and medical images~\cite{DBLP:conf/miccai/SaabDGRSRR19,Saab2020WeakSA,DBLP:journals/patterns/DunnmonRSKMSGLL20}.

\paragraph{Others.} 
Apart from aforementioned areas, PWS are also used in software engineering~\cite{rao2021search}, mobile sensing~\cite{furst2020transport,khattar2019multi}, E-commerce platforms~\cite{mathewdefraudnet,zhang2021fraud}, and multi-agent systems~\cite{DBLP:conf/iclr/ZhanZYSL19}.


==> 04-toolkit.tex <==
\section{Systems}
Snorkel~\cite{ratner2017snorkel}

Tagruler

Knodle~\cite{sedova2021knodle}: modularizing WS pipelines

SPEAR~\cite{abhishek2021spear}: Open source toolkit for semi-supervised WS.

skweak~\cite{skweak}: facilitate the use of weak supervision for NLP tasks such as text classification and sequence labelling.

TagRuler~\cite{tagruler}

==> modifiednasa.tex <==
\iffalse(J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)
\begin{algorithm}
\caption{Multilevel Nested Averaging Stochastic Gradient Method}
\begin{algorithmic}
	\STATE \textbf{Input:} A positive integer sequence $\{\beta_k\}_{k \ge 0}$ and initial points $x^0 \in X, \quad w_i^0 \in \bbr^{d_i} \quad 1 \le i \le T$
    \FOR{$k = 0,1, 2, \dots, $}
        \STATE  1. Compute
\begin{equation}
\label{def_uk}
u^k = \argmin_{y \in X}\  \left\{\langle z^k, y-x^k \rangle + \frac{\beta_k}{2} \|y-x^k\|^2\right\},
\end{equation}
stochastic gradients $J_i^{k+1}$, and function values $G_{i}^{k+1}$ at $w_{i+1}^k$ for $i=\{1,\dots,T\}$, by denoting $w^k_{T+1} = x^k$.

\STATE 2. Set
\begin{align}
x^{k+1} & = (1 - \tau_k)x^k + \tau_k u^k \label{def_xk_new}\\
z^{k+1} & = (1 - \tau_k)z^k + \tau_k \prod_{i=1}^TJ_{T+1-i}^{k+1} \label{def_zk_new}\\
w_i^{k+1} & = (1 - \tau_k)w_i^k + \tau_k G_i^{k+1} + (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k), \qquad  1\leq i \leq T \label{def_wk_new}
%(1-b\tau_k)w_T^k + b\tau_kG_T^{k+1} + J_T^{k+1}(x^{k+1}-x^k) &~~~ i=T
\end{align}
    \ENDFOR
    \STATE \textbf{Output:}
\end{algorithmic}
\label{alg:modifiednasa}
\end{algorithm}
\fi

\section{Multi-level Nested Linearized Averaging Stochastic Gradient \\ Method}\label{sec:modifiednasa}
In this section, we present a linearized variant of \cref{alg:originalnasa} which can achieve the best known rate of convergence for problem \eqnok{eq:mainprob} for any $T\geq 1$, under Assumptions~\ref{fi_lips} and~\ref{assumption:original_nasa_assumption}. Indeed, when $T>2$, we have accumulated errors in estimating the inner function values. Hence, in~\cref{alg:originalnasa} we use mini-batch sampling in \eqnok{def_wi} to reduce the noise associated with the stochastic function values. However, this increases the sample complexity of the algorithm. To resolve this issue, instead of using the point estimates of $f_i$'s, we use their stochastic linear approximations in \eqnok{def_wi_new}. This modification reduces the bias error in estimating the inner function values which together with a refined convergence analysis enable us to obtain a sample complexity of ${\cal O}_T(1/\epsilon^4)$ with \cref{alg:modifiednasa}, for any $T\geq 1$ without using any mini-batches. \textcolor{black}{Furthermore,~\cref{alg:modifiednasa} works with any constant choice of step-size parameter $\beta$ (independent of the problem parameters), making it easy to implement.} As mentioned previously,~\cref{alg:modifiednasa} is motivated by the algorithm in \cite{rusz20} proposed for solving nonsmooth multi-level stochastic composition problems. However, \cite{rusz20} assumes that all functions $f_i$ explicitly depend on the decision variable $x$ which makes the composition function a variant of the general case in \eqnok{eq:mainprob}. It is also worth mentioning that other linearization techniques have been used in~\cite{duchi2018stochastic, davis2019stochastic} in estimating the stochastic inner function values for weakly convex two-level composition problems.

 %By considering \eqnok{def_wi_new}, our \cref{alg:modifiednasa} becomes similar to a recent work by \cite{rusz20} proposed for solving nonsmooth multi-level stochastic composition problems. However, the finite-time convergence analysis of \cite{rusz20} is not complete and thus, we are unable to compare our results in this regard.}




\begin{algorithm}
\caption{Multi-level Nested Linearized Averaging Stochastic Gradient Method}
\begin{algorithmic}
\STATE Set $b_k=1$ in Algorithm~\ref{alg:originalnasa} and replace \eqnok{def_wi} with
\beq\label{def_wi_new}
w_i^{k+1} = (1 - \tau_k)w_i^k + \tau_k G_i^{k+1} + (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k), \qquad  1\leq i \leq T.
\eeq
\end{algorithmic}
\label{alg:modifiednasa}
\end{algorithm}

To establish the rate of convergence of \cref{alg:modifiednasa}, we first need the next result which provides the recursion on the errors in estimating the inner function values.
\begin{lemma}\label{new_nasa_lemma_fn_w_error}
Let $\{x^k\}_{k \ge 0}$ and $\{w^k_i\}_{k \ge 0}$ be generated by~\cref{alg:modifiednasa}. Define, for $1\leq i\leq T$,
\begin{align}
e_i^{k+1}:= f_i(w_{i+1}^k) - G_i^{k+1},&~\hat{e_i}^{k+1}: = \nabla f_i(w_{i+1}^k) - J_i^{k+1},\label{new_nasa_errors}\\
\hat A_{k,i}  := f_i(w_{i+1}^{k+1}) - f_i(w_{i+1}^k&) - \nabla f_i(w_{i+1}^k)^\top (w_{i+1}^{k+1}-w_{i+1}^k) \label{new_nasa_A_ki}.
%A_{k,T} & := f_T(x^{k+1}) - f_T(x^k) - \nabla f_T(x^k)(x^{k+1}-x^k). \label{new_nasa_A_kT}
\end{align}
\begin{itemize}[leftmargin=0.2in]
\item [a)] Under~\cref{fi_lips}, we have, for~$1 \leq i \leq T$,
\begin{align}
 & \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2  \leq (1-\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2 + \tau_k^2\|e_i^{k+1}\|^2 + \dot{r}_i^{k+1} \notag\\
& + \left[8 L_{ f_i}^2+ L_{\nabla f_i} \|f_i(w_{i+1}^k) - w_i^k\|+ \| \hat{e_i}^{k+1}\|^2\right] \|w_{i+1}^{k+1}-w_{i+1}^k\|^2, \label{new_nasa_fn_w_error_i}\\
\dot{r}^{k+1}_i &:=2\tau_k\langle e_i^{k+1}, \hat A_{k,i} + (1-\tau_k)(f_i(w_{i+1}^k) - w_i^k) + (\hat{e_i}^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)\rangle  \nonumber \\ 
&+2\langle (\hat{e_i}^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k), \hat A_{k,i}+(1-\tau_k)(f_i(w_{i+1}^k)-w_i^k)\rangle.\label{new_nasa_r_i}
\end{align}

\item [b)] Furthermore, we have for $1\leq i \leq T$, $\| w_i^{k+1} - w_i^k\|^2 \leq$
\begin{align*}
& \tau_k^2\left[2\| f_i(w_{i+1}^k) - w_i^k\|^2 + \|e_i^{k+1}\|^2 + \frac{2}{\tau_k^2}\|J_i^{k+1}\|^2 \| w_{i+1}^{k+1} - w_{i+1}^k \|^2\right]+2 \ddot{r}^{k+1}_i,
\end{align*}
where $ \ddot{r}^{k+1}_i := \tau_k \langle -e_i^{k+1}, \tau_k(f_i(w_{i+1}^k) - w_i^k) + (J_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\rangle.$
\end{itemize}
\end{lemma}
\begin{proof}
We first prove part a). 

When $1\leq i < T$, by definition of $\hat A_{k,i}, \hat{e_i}^{k+1},G_i^{k+1},w_i^{k+1}$, and $\dot{r}_i^{k+1}$, we have
\begin{align}
    & \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 \notag\\ 
    = & \|\hat A_{k,i} + f_i(w_{i+1}^k) + \nabla f_i(w_{i+1}^k)^\top (w_{i+1}^{k+1}-w_{i+1}^k) \notag  \\
    &\qquad- (1-\tau_k)w_i^k - \tau_kG_i^{k+1} - (J_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\|^2 \notag\\  
    = & \|\hat A_{k,i} + (\widehat{e_i}^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k) + (1-\tau_k)(f_i(w_{i+1}^k) - w_i^k) + \tau_ke_i^{k+1}\|^2 \label{fi_wi_modified_nasa}\\  
    =& \|(\widehat{e_i}^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\|^2 + \|\hat A_{k,i} + (1-\tau_k)(f_i(w_{i+1}^k)-w_i^k)\|^2 + \tau_k^2\|e_i^{k+1}\|^2 + \dot{r}_i^{k+1} \notag\\  
    \leq & \|\hat A_{k,i} + (1-\tau_k)(f_i(w_{i+1}^k) - w_i^k)\|^2 +\tau_k^2\|e_i^{k+1}\|^2 + \dot{r}_i^{k+1} + \|\widehat{e_i}^{k+1}\|^2\|w_{i+1}^{k+1}-w_{i+1}^k\|^2\notag\\
    \leq & (1-\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2+\|\hat A_{k,i}\|^2+ 2(1-\tau_k)\langle \hat A_{k,i}, f_i(w_{i+1}^k) - w_i^k\rangle +\tau_k^2\|e_i^{k+1}\|^2 \notag\\
    &\qquad + \dot{r}_i^{k+1}+ \|\widehat{e_i}^{k+1}\|^2\|w_{i+1}^{k+1}-w_{i+1}^k\|^2.\label{fi_wi_modified_nasa2}
\end{align}
Now, noting that under~\cref{fi_lips}, we have 
\beq\label{Ak_bnd}
\|\hat A_{k,i}\| \le \frac{1}{2}\min\left\{4 L_{f_i}\|w_{i+1}^{k+1}-w_{i+1}^k\|, L_{\nabla f_i}\|w_{i+1}^{k+1}-w_{i+1}^k\|^2 \right\},
\eeq
and using Cauchy–Schwarz inequality in \eqnok{fi_wi_modified_nasa2}, we obtain \cref{new_nasa_fn_w_error_i}.

To show part b), noting definition of \cref{def_wi_new} and \cref{new_nasa_errors}, Cauchy-Schwartz and Young's inequality, for $1\leq i \leq T$,
\begin{align*}
    &\| w_i^{k+1} - w_i^k\|^2 \\
     =& \| \tau_k(G_i^{k+1}-w_i^k) + (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)\|^2 \\  = &\tau_k^2\|G_i^{k+1} - w_i^k\|^2 + \| (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)\|^2 + 2\tau_k\langle G_i^{k+1} - w_i^k, (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)\rangle \\
    \leq & \tau_k^2 \| G_i^{k+1} - w_i^k\|^2 + 2\|J_i^{k+1}\|^2 \|w_{i+1}^{k+1} - w_{i+1}^{k}\|^2 + \tau_k^2 \|f_i(w_{i+1}^k) - w_i^k\|^2 \\
     &+ 2\tau_k\langle -e_i^{k+1}, (J_i^{k+1})^\top(w_{i+1}^{k+1} - w_{i+1}^k)\rangle  \\
     =& 2\tau_k^2 \| f_i(w_{i+1}^k) - w_i^k\|^2 + \tau_k^2 \|e_i^{k+1}\|^2 + 2\|J_i^{k+1}\|^2 \|w_{i+1}^{k+1} - w_{i+1}^k\|^2 \\  &+ 2\tau_k \langle -e_i^{k+1}, \tau_k(f_i(w_{i+1}^k) - w_i^k) + (J_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\rangle.
\end{align*}
\end{proof}


\noindent In the next result, we show how the moments of $\|w_i^{k+1} - w_i^k\|$ decrease in the corresponding order of $\tau_k$. This is a crucial step on bounding the errors in estimating the inner function values.

\begin{lemma}\label{moment_bounds}
Under~\cref{fi_lips}, \cref{assumption:original_nasa_assumption}, for $1\leq i \leq T$, and with the choice of $\tau_0=1$ (for simplicity), we have
\begin{align}
&\mathbb{E}[ \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2  | \mathscr{F}_k] \leq  \sigma_{G_i}^2+(4L_{f_i}^2+ \hat \sigma_{J_i}^2)c_{i+1} ,\label{fi-wi_bound}\\
&\mathbb{E}[\|w_i^{k+1} - w_i^k\|^2 | \mathscr{F}_k] \leq c_i~\tau^2_k,  \label{new_nasa_conditional_expectation_w_T_second_power}
\end{align}
where, for $1 \le i \le T$,
\begin{align}
c_i := 3 \sigma_{G_T}^2+2(4L_{f_T}^2+\hat \sigma_{J_T}^2+\sigma_{J_T}^2) c_{i+1},~~~\text{with}~~~ c_{T+1} := \left(\prod_{i=1}^T\sigma_{J_i}^2\right) \beta^{-2}.\label{def_ci}
\end{align}
\end{lemma}

\vgap

\begin{proof}
Recall the definitions of $\hat A_{k,i}, e_i^{k+1}, \hat{e}_i^{k+1}$ and, for $1\leq i\leq T$, define
\begin{align}
    D_{k,i} := \hat A_{k,i} + \tau_ke_i^{k+1} + \hat{e}_i^{k+1}(w_{i+1}^{k+1}-w_{i+1}^k).\label{new_nasa_D_ki}
\end{align}
Then, by \eqnok{fi_wi_modified_nasa}, for $1\leq i\leq T$, we have
\begin{align}
    f_i(w_{i+1}^{k+1}) - w_i^{k+1} & = (1-\tau_k)(f_i(w_{i+1}^k)-w_i^k) + D_{k,i},\label{new_nasa_fi_w_i_D_ki}
\end{align}
which together with the convexity of $\|\cdot\|^2$, imply that
\begin{align}
\|f_i(w_{i+1}^{k+1})-w_i^{k+1}\|^2 &\leq (1-\tau_k)\|f_i(w_{i+1}^{k})-w_i^k\|^2 + \frac{1}{\tau_k}\|D_{k,i}\|^2. \label{fi-wi_Dki}\
\end{align}
Moreover, we have
\begin{align}
\|D_{k,i}\|^2 &= \|\hat A_{k,i}\|^2 + \tau_k^2 \|e_i^{k+1}\|^2 + \|(\hat{e}_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\|^2 +2 r'_{k,i}, \label{Dki_squared}\\
r'_{k,i} &= \langle \hat A_{k,i},\tau_k e_i^{k+1}+(\hat{e}_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k) \rangle + \tau_k \langle e_i^{k+1}, (\hat{e}_i^{k+1})^\top(w_{i+1}^{k+1}-w_{i+1}^k)\rangle,\nonumber
\end{align}
which together with the fact that $\mathbb{E}[r'_{k,i}| \mathscr{F}_k]=0$ under~\cref{assumption:original_nasa_assumption}, imply that
\begin{align}
\mathbb{E}[\|D_{k,i}\|^2| \mathscr{F}_k] &= \mathbb{E}[\|\hat A_{k,i}\|^2| \mathscr{F}_k] + \tau_k^2 \mathbb{E}[\|e_i^{k+1}\|^2| \mathscr{F}_k] +
\mathbb{E}[\|\hat{e}_i^{k+1}(w_{i+1}^{k+1}-w_{i+1}^k)\|^2| \mathscr{F}_k] \nonumber\\
&\le \tau_k^2 \mathbb{E}[\|e_i^{k+1}\|^2| \mathscr{F}_k] +
\left(4L_{f_i}^2+\mathbb{E}[\|\hat{e}_i^{k+1}\|^2|\mathscr{F}_k]\right) \mathbb{E}[\|w_{i+1}^{k+1}-w_{i+1}^k\|^2| \mathscr{F}_k],\label{exp_Dki_squared}
\end{align}
where the second inequality follows from \eqnok{Ak_bnd}.
Hence, noting \eqnok{dk_bnd}, $w_{T+1}^{k} =x^k$,  we have
\begin{align*}
    \mathbb{E}[\|D_{k,T}\|^2 | \mathscr{F}_k] & \leq \tau_k^2\left[\sigma_{G_T}^2+\left(4L_{f_T}^2+\hat \sigma_{J_i}^2\right)\left(\prod_{i=1}^T\sigma_{J_i}^2\right) \beta^{-2}\right].
\end{align*}
Using \eqnok{fi-wi_Dki} with $i=T$, the above inequality, and~\cref{Gamma_lemma} with the choice of $\tau_0=1$, we have
\beq\label{fT_squared_bnd}
\mathbb{E}[\|f_T(x^{k})-w_T^{k}\|^2 | \mathscr{F}_k] \leq \sigma_{G_T}^2+\left(4L_{f_T}^2+\hat \sigma_{J_i}^2\right)\left(\prod_{i=1}^T\sigma_{J_i}^2\right) \beta^{-2}.
\eeq
Moreover, by \cref{new_nasa_lemma_fn_w_error}.b) and under \cref{assumption:original_nasa_assumption}, we have $\mathbb{E}[\|w_{i+1}^{k+1}-w_i^k\|^2 | \mathscr{F}_k] \le $
\beq\label{wi_ineq}
 \tau_k^2\mathbb{E}\left[2\| f_i(w_{i+1}^k) - w_i^k\|^2 + \|e_i^{k+1}\|^2 + \frac{2}{\tau_k^2}\|J_i^{k+1}\|^2 \| w_{i+1}^{k+1} - w_{i+1}^k \|^2 \Big| \mathscr{F}_k\right],
\eeq
implying that
\beq
\mathbb{E}[\|w_T^{k+1}-w_T^k\|^2 | \mathscr{F}_k] \le \tau_k^2\left[3 \sigma_{G_T}^2+2(4L_{f_T}^2+\hat \sigma_{J_T}^2+\sigma_{J_T}^2)\left(\prod_{i=1}^T\sigma_{J_i}^2\right) \beta^{-2}\right].
\eeq
This completes the proof of~\cref{fi-wi_bound} and \cref{new_nasa_conditional_expectation_w_T_second_power} when $i=T$. We now use backward induction to complete the proof.  By the above result, the base case of $i=T$ holds. Assume that $\mathbb{E}[\|w_{i+1}^{k+1}-w_{i+1}^k\|^2|\mathscr{F}_k] \leq c_{i+1}\tau_k^2$ for some $1\leq i < T$. Hence, by \cref{Dki_squared} and under~\cref{assumption:original_nasa_assumption}, we have
\begin{align*}
\mathbb{E}[\|D_{k,i}\|^2|\mathscr{F}_k] \leq \tau_k^2[\sigma_{G_i}^2+(4L_{f_i}^2+ \hat \sigma_{J_i}^2)c_{i+1}],
\end{align*}
which together with \cref{Gamma_lemma}, imply that
\begin{align*}
    \mathbb{E}[\|f_i(w_{i+1}^{k})-w_i^{k}\|^2 | \mathscr{F}_k] \leq \sigma_{G_i}^2+(4L_{f_i}^2+ \hat \sigma_{J_i}^2)c_{i+1}].
    %\|f_i(w_{i+1}^0) - w_i^0\|^2 + 16L_{f_i}^2\tilde{c}_{i+1} + 8\sigma_{G_i}^2 + 8\hat{\sigma}_i^2\tilde{c}_{i+1}.
\end{align*}
Thus, by \cref{wi_ineq}, we obtain
\begin{align*}
    \mathbb{E}[\|w_i^{k+1}-w_i^k\|^2|\mathscr{F}_k] & \leq \tau_k^2[3\sigma_{G_i}^2+2(4L_{f_i}^2+ \hat \sigma_{J_i}^2+\sigma^2_{J_i})c_{i+1}],
\end{align*}
which together with the definition of $c_i$ in \eqnok{def_ci}, complete the proof.
\end{proof}

\vgap

\noindent The next result is the counterpart of \cref{original_nasa_merit_function_lemma} for \cref{alg:modifiednasa}.

\begin{lemma} \label{new_nasa_merit_function_lemma}
Recall the definition of the merit function in~\cref{merit_function}. Define $w^k:= (w_1^k,\dots,w_T^k)$ for $k \geq 0$. Let $\{x^k,z^k,u^k,w_1^k,\dots,w_T^k\}_{k \geq 0}$ be the sequence generated by~\cref{alg:modifiednasa}. Suppose that
\begin{align}
    %\max_{2 \leq j \leq T}C_j^2 & \leq \frac{(\beta-\lambda )}{T}(\gamma_i - \lambda) \label{new_nasa_merit_function_upperbound_assumption}
\gamma_1 \ge \lambda >0, \quad \beta >\lambda, \quad    (\beta-\lambda ) (\gamma_j - \lambda) \ge 4 T C_j^2 , \qquad  j \in \{2,\ldots,T\}, \label{new_nasa_merit_function_upperbound_assumption}
\end{align}
where $C_j$'s are defined in Lemma~\ref{FZ_difference}. Then, under~\cref{fi_lips} and~\cref{assumption:original_nasa_assumption}, we have
\begin{align} \label{modified_nasa_main_rec}
&\lambda \sum_{k=0}^{N-1}\tau_k\left[\|d^k\|^2 + \sum_{i=1}^{T-1}\|f_i(w_{i+1}^k) - w_i^k\|^2 + \|f_T(x^k) - w_T^k\|^2 \right] \notag\\
&\leq W_\gamma(x^0,z^0,w^0) + \sum_{k=0}^{N-1} \hat{R}^{k+1},
\end{align}
where, for any $k \geq 0$,
\begin{align}
\hat{R}^{k+1} & := \left(\sum_{i=1}^T\gamma_i\hat{r}_i^{k+1}\right) + \frac{\tau_k^2}{2}\left[(L_{\nabla F} + L_{\nabla \eta} \right] + \tau_k\langle d^k,\Delta_k\rangle + \frac{L_{\nabla \eta}}{2}\|z^{k+1} - z^k\|^2, \label{def_Rhatk}\\
    \hat{r}_i^{k+1} & = \left[8 L_{ f_i}^2+ L_{\nabla f_i} \|f_i(w_{i+1}^k) - w_i^k\|+ \| \hat{e_i}^{k+1}\|^2\right] \|w_{i+1}^{k+1}-w_{i+1}^k\|^2 \notag\\
    &+\tau_k^2\|e_i^{k+1}\|^2 + \dot{r}_i^{k+1},\notag
\end{align}
and $\Delta_k$ and $\dot{r}_i^{k+1}$ are, respectively, defined in \eqnok{def_deltak} and \eqnok{new_nasa_r_i}.
Furthermore, notice that~\cref{new_nasa_merit_function_upperbound_assumption} is satisfied, when we pick
{\color{black}
\begin{align}\label{new_nasa_merit_function_gamma_choice}
\gamma_1 = \lambda = \sqrt{T}, \qquad \beta = 2\sqrt{T}, \qquad  \gamma_j = \sqrt{T}(1  + 4 C_j^2) \qquad 2\le j \le T.
\end{align}
}




\end{lemma}


\begin{proof}
Noting \cref{new_nasa_lemma_fn_w_error} and definition of $\hat{r}_i^{k+1}$, we have, $\forall i \in \{1,2,\ldots, T\},$
\begin{align*}
    \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 - \|f_i(w_{i+1}^k) - w_i^k\|^2 & \leq -\tau_k\|f_i(w_{i+1}^k) - w_i^k\|^2 + \hat{r}_i^{k+1}.
 %   \|f_T(x^{k+1}) - w_T^{k+1}\|^2 - \|f_T(x^k) - w_T^k\|^2 & \leq -\tau_k\|f_T(x^k) - w_T^k\|^2 + \hat{r}_T^{k+1},
\end{align*}
Combining the above inequalities with \eqnok{F_lips}, \eqnok{eta_lips}, noting definition of the merit function in \eqnok{merit_function}, and in the view of \cref{FZ_difference}, we obtain
\begin{align*}
    & W_\gamma(x^{k+1},z^{k+1},w^{k+1}) - W_\gamma(x^k,z^k,w^k) \\ \leq & -\beta \tau_k\|d^k\|^2 + \sum_{j=2}^{T-1}\tau_kC_j\|d^k\| \|f_j(w_{j+1}^k)-w_j^k\| + \tau_kC_T\|d^k\|\|f_T(x^k)-w_T^k\| \\  -& \sum_{j=1}^{T-1}\gamma_j\tau_k\|f_j(w_{j+1}^k) - w_j^k\|^2 - \gamma_T\tau_k\|f_T(x^k) - w_T^k\|^2 + \hat{R}^{k+1}
\end{align*}
{\color{black}Now if condition \cref{new_nasa_merit_function_upperbound_assumption} holds, for any $i \in \{1,\ldots,T\}$, we have
 \begin{align*}
&-\frac{\beta}{T}\|d^k\|^2 + C_i\|d^k\| \|f_i(w_{i+1}^k)-w_i^k\|- \gamma_i\|f_i(w_{i+1}^k) - w_i^k\|^2 \\
\le & -\lambda \big[\frac{1}{T}\|d^k\|^2 + \|f_i(w_{i+1}^k) - w_i^k\|^2\big].
\end{align*}
Combining the above inequalities, we obtain
\begin{align*}
& W_\gamma(x^{k+1},z^{k+1},w^{k+1}) - W_\gamma(x^k,z^k,w^k) \\
 \leq& -\lambda \tau_k \Big[\|d^k\|^2 + \sum_{j=1}^{T-1}\|f_j(w_{j+1}^k) - w_j^k\|^2 + \|f_T(x^k)-w_T^k\|^2\Big] + \hat{R}^{k+1}.
\end{align*}
}
Thus, by summing up the above inequalities and re-arranging the terms, we obtain \eqnok{modified_nasa_main_rec}. Finally, it is easy to see that \cref{new_nasa_merit_function_upperbound_assumption} holds, by picking the parameters as in~\cref{new_nasa_merit_function_gamma_choice}.
\end{proof}

\vgap

In the next result, we show the error terms in the right hand side of \eqnok{modified_nasa_main_rec} is bounded in the order of $\sum_{k=1}^N \tau_k^2$ in expectation.

\begin{proposition} \label{new_nasa_big_proposition}
Let $\hat{R}^k$ be defined in \eqnok{def_Rhatk}. The, under \cref{assumption:original_nasa_assumption}, we have
\[
\mathbb{E}[\hat{R}^{k+1} | \mathscr{F}_k] \leq \hat{\sigma}^2 \tau_k^2, \qquad \forall k \geq 1, 
\]
where 
\begin{align}
    \hat{\sigma}^2 & := \sum_{i=1}^{T}\gamma_i\left(\left[8L_{f_i}^2+L_{\nabla f_i}\sqrt{\sigma_{G_i}^2+(4L_{f_i}^2+ \hat \sigma_{J_i}^2)c_{i+1}}+ \hat \sigma_{J_i}^2 \right]{c}_{i+1} + \sigma_{G_i}^2\right) \notag\\
    &+  \frac{1}{2\beta^2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right)[(1+4\beta^2) L_{\nabla \eta}+L_{\nabla F}]. \label{new_nasa_big_proposition_sigma_squared}
\end{align}

\end{proposition}

\begin{proof}
Under \cref{assumption:original_nasa_assumption}, we have, for $1 \leq i \leq T$,
\[
\mathbb{E}[\Delta_k | \mathscr{F}_k] = 0, \quad \mathbb{E}[\dot{r}_i^{k+1}|\mathscr{F}_k] = 0, \quad \mathbb{E}[ \| \hat{e_i}^{k+1}\|^2|\mathscr{F}_k] \le \sigma_{G_i}^2, \quad \mathbb{E}[ \| {e_i}^{k+1}\|^2|\mathscr{F}_k] \le \hat \sigma_{J_i}^2.
\]
Moreover, by \cref{moment_bounds} and Holder's inequality, we have $\mathbb{E}[\|w_i^{k+1} - w_i^k\|^2 | \mathscr{F}_k] \leq c_i~\tau^2_k$ and
\begin{align*}
&\mathbb{E}[ \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\| \|w_i^{k+1} - w_i^k\|^2| \mathscr{F}_k] \\ 
\le& \left(\mathbb{E}[ \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 | \mathscr{F}_k]\right)^{\frac12} \mathbb{E}[\|w_i^{k+1} - w_i^k\|^2 | \mathscr{F}_k]\\
\leq&  c_i \sqrt{\sigma_{G_i}^2+(4L_{f_i}^2+ \hat \sigma_{J_i}^2)c_{i+1}} \tau^2_k
\end{align*}
The result then follows by noting the definition of $\hat \sigma^2$ in \cref{new_nasa_big_proposition_sigma_squared}
\end{proof}

\vgap

We are now ready to state the convergence rates via the following theorem.
\begin{theorem}\label{optimal_theorem}
Suppose that $\{ x^k, z^k \}_{k\geq 0}$ are generated by~\cref{alg:modifiednasa}, and~\cref{fi_lips} and~\cref{assumption:original_nasa_assumption} hold. Also assume the parameters satisfy~\cref{new_nasa_merit_function_gamma_choice} and the step sizes $\{\tau_k\}$ satisfy \eqnok{gamma_condition}.
\begin{itemize}
\item [(a)] The results in parts a) and b) of \cref{nasa_main_theorem} still hold by replacing $\sigma^2$ by $\hat \sigma^2$.

\item [b)] If $\tau_k$ is set as in \eqnok{def_tau}, the results of part c) of \cref{nasa_main_theorem} also hold with $\hat \sigma^2$ replacing $\sigma^2$.
\end{itemize}

\end{theorem}

\begin{proof}
The proof follows from the same arguments as in the proof of \cref{nasa_main_theorem} by noticing \eqnok{modified_nasa_main_rec}, and \cref{new_nasa_big_proposition}, hence, we skip the details.

\end{proof}
\begin{remark}\label{remark:rmk2}
Note that \cref{alg:modifiednasa} does not use a mini-batch of samples in any iteration. Thus, \eqnok{nasa_main_theorem3} (in which $\sigma^2$ is replaced by $\hat \sigma^2$) implies that the total sample complexity of \cref{alg:modifiednasa} for finding an $\epsilon$-stationary point of \cref{eq:mainprob}, is bounded by ${\cal O}(c^T T^4/\epsilon^4)={\cal O}_T(1/\epsilon^4)$ which is better in the order of magnitude than the complexity bound of \cref{alg:originalnasa}. Furthermore, this bound matches the complexity bound obtained in \cite{GhaRuswan20} for the two-level composite problem which in turn is in the same order for single-level smooth stochastic optimization. Finally, it is worth noting that this complexity bound for \cref{alg:modifiednasa} is obtained without assuming boundedness of the feasible set or any dependence of the parameter $\beta$ on Lipschitz constants. Indeed, $\beta$ can be set to any positive number in the order of ${\cal O}(\sqrt{T})$ due to \eqnok{new_nasa_merit_function_gamma_choice}, and $\tau_k$ depends only on the total number of iterations $N$ due to \eqnok{def_tau}. This makes \cref{alg:modifiednasa} parameter-free and easy to implement.
\end{remark}

%\clearpage
%{
%\color{blue}{
%Finally, observe $\max_{1 \leq i \leq T}L_i = \mathcal{O}(T), \lambda = \mathcal{O}(1), \beta = \mathcal{O}(T)$, so $L_{\nabla \eta} = \mathcal{O}(T)$. Hence, $c_i, \tilde{c}_i = \mathcal{O}(\rho^{T-i})$ for $1 \leq i \leq T$ for some constant $\rho > 0$ that depends on the Lipschitz constants and parameters in assumption \ref{new_nasa_assumption}. Hence, $\sigma^2 = \mathcal{O}(\rho^T)$.
%Hence, we have
%\begin{align}
%    \mathbb{E}[V(x^R,z^R)] & = \mathcal{O}\left(\frac{T^3\rho^T}{\sqrt{N}}\right) \label{new_nasa_big_theorem_complexity_lyaponuv} \\ \mathbb{E}[\|f_i(w_{i+1}^R) - w_i^R\|^2] & = \mathcal{O}\left(\frac{T\rho^T}{\sqrt{N}}\right) \quad \text{ for } i = 1, \dots, T \label{new_nasa_big_theorem_complexity_fiwi}  \\ \mathbb{E}[\|f_T(x^R) - w_T^R\|^2] & = \mathcal{O}\left(\frac{T\rho^T}{\sqrt{N}}\right) \label{new_nasa_big_theorem_complexity_fTwT}
%\end{align}
%}
%}






==> originalnasa.tex <==
\section{Multi-level Nested Averaging Stochastic Gradient Method}\label{sec:originalnasa}
In this section, we present our first algorithm for solving problem \eqnok{eq:mainprob}. As mentioned in~\cref{sec:intro}, the previously proposed stochastic gradient-type methods suffer in terms of the convergence rates when applied for solving this problem~\cite{yang2019multi-level}. The main reason is the increased bias when estimating the stochastic gradient of $F$, for $T \ge 2$. Our proposed algorithm has a multi-level structure -- in addition to estimating the gradient of $F$, we also estimate the values of inner functions $f_i$ by a mini-batch moving average technique, extending the approach in~\cite{GhaRuswan20} for any $T>1$. This will enable us to provide an algorithm with improved convergence rates to the stationary points compared to the prior work~\cite{yang2019multi-level}. Our approach is formally presented in~\cref{alg:originalnasa}.
%\subsection*{Algorithm}
\begin{algorithm}[ht]
\caption{Multi-level Nested Averaging Stochastic Gradient Method}
\begin{algorithmic}
	\STATE \textbf{Input:} \textcolor{black}{Positive integer sequences $\{b_k,\tau_k\}_{k \ge 0}$, step-size parameter $\beta$, and initial points $x^0 \in  X, \quad z^0 \in \bbr^{d_T}, \qquad w_i^0 \in \bbr^{d_{i-1}} \quad 1 \le i \le T$, and a probability mass function $P_R(\cdot)$ supported over $\{1,2,\ldots,N\}$, where $N$ is the number of iterations}.
	 \STATE  0. Generate a random integer number $R$ according to $P_R(\cdot)$.
    \FOR{$k = 0,1, 2, \dots, R$}
        \STATE  1. Compute
\begin{equation}
\label{def_uk}
u^k = \argmin_{y \in X}\  \left\{\langle z^k, y-x^k \rangle + \frac{\beta}{2} \|y-x^k\|^2\right\},
\end{equation}
stochastic gradients $J_i^{k+1}$, and function values $G_{i,j}^{k+1}$ at $w_{i+1}^k$ for $i=\{1,\dots,T\}, j=\{1,\dots,b_k\}$ by denoting $w_{T+1}^k \equiv x^k$.

\STATE 2. Set
\begin{align}
x^{k+1}  &= (1 - \tau_k)x^k + \tau_k u^k, \label{def_xk}\\
z^{k+1}  &= (1 - \tau_k)z^k + \tau_k \prod_{i=1}^TJ_{T+1-i}^{k+1}, \label{def_zk}\\
w_i^{k+1} &= (1 - \tau_k)w_i^k + \tau_k \bar G_i^{k+1}, \qquad 1 \le i \le T,\label{def_wi}
\end{align}
where
\beq\label{def_barG}
\bar G_i^{k+1} = \frac{1}{b_k}\sum_{j=1}^{b_k} G_{i,j}^{k+1}.
\eeq
    \ENDFOR
    \STATE \textbf{Output:} $(x^R, z^R, w_1^R, \ldots, w_T^R)$.
\end{algorithmic}
\label{alg:originalnasa}
\end{algorithm}

We now add a few remarks about \cref{alg:originalnasa}. First, note that at each iteration of this algorithm, we update the triple $(x^k, \{w^k\}_{i=1}^T, z^k)$, which are the convex combinations of the solutions to subproblem \eqnok{def_uk}, the estimates of inner function values $f_i$, and the stochastic gradient of $F$ at these points, respectively. It should be mentioned that we do not need to estimate the values of the outer function $f_1$. However, we include $w^k_1$ for the sake of completeness. Second, when $T=2$ and $b_k=1$, this algorithm reduces to the NASA algorithm presented in \cite{GhaRuswan20}. Indeed, \cref{alg:originalnasa} is a direct generalization of the NASA method to the multi-level case $T \ge 3$. However, to prove convergence of \cref{alg:originalnasa}, we need to take a batch of samples in each iteration to reduce the noise associated with estimation of the inner function values, when $T >2$. We now provide our convergence analysis for~\cref{alg:originalnasa}. To do so, we define the following filtration, $$\mathscr{F}_k:=\sigma(\{x^0,\ldots, x^k, z^0,\ldots, z^k, w_1^0,\ldots,w_1^k, \dots, w_T^0, \dots, w_T^k, u^0,\ldots, u^k\}).$$
Next, we state our main assumptions on the individual functions and the stochastic first-order oracle we use.

\begin{assumption}\label{fi_lips}
All functions $f_1,\dots,f_T$ and their derivatives are Lipschitz continuous with Lipschitz constants $L_{f_i}$ and $L_{\nabla f_i}$, respectively.
\end{assumption}
\begin{assumption}\label{assumption:original_nasa_assumption}
Denote $w_{T+1}^k \equiv x^k$. For each $k$, $w_{i+1}^k$ being the input, the stochastic oracle outputs $G_{i}^{k+1} \in \mathbb{R}^{d_i}$ and $J_{i}^{k+1} \in \mathbb{R}^{d_i \times d_{i-1}}$ such that
\begin{enumerate}
\item For $i \in \{1,\ldots,T\}$, we have $\mathbb{E}[J_{i}^{k+1}| \mathscr{F}_k] = \nabla f_i(w_{i+1}^k),~\text{and}~~\mathbb{E}[G_{i}^{k+1}| \mathscr{F}_k] = f_i(w_{i+1}^k)$.
\item For $i \in \{1,\ldots,T\}$, we have $\mathbb{E}[\| G_i^{k+1} - f_i(w_{i+1}^k) \|^2 | \mathscr{F}_k] \leq \sigma_{G_i}^2,\mathbb{E}[\| J_i^{k+1} - \nabla f_i(w_{i+1}^k) \|^2 | \mathscr{F}_k] \leq \hat \sigma_{J_i}^2,~\text{and}~~\mathbb{E}[\|J_i^{k+1}\|^2 | \mathscr{F}_k] \leq \sigma_{J_i}^2$. Here $\|\cdot\|$ denotes the Euclidean norm for vectors and the Frobenius norm for matrices.
\item Given $\mathscr{F}_k$, the outputs of the stochastic oracle at each level $i$, $G_{i}^{k+1}$ and $J_{i}^{k+1}$, are independent.
\item Given $\mathscr{F}_k$, the outputs of the stochastic oracle are independent between levels i.e., $\{G_{i}^{k+1}\}_{i=1,\ldots,T}$ are independent and so are $\{J_{i}^{k+1}\}_{i=1,\ldots,T}$.
%\item $\mathbb{E}\left[\prod_{i=1}^T J_{T-i+1}^{k+1} | \mathscr{F}_k\right]=\nabla f_T(x^k) \prod_{i=2}^T \nabla f_{T+1-i}(w^k_{T+2-i})$.

%\item $\tilde{f_i}(w_{i+1}^k) = F_i(w_{i+1}^k,\xi_i) = G_{i}^{k+1} \quad i \leq T-1 $
%\item $ \tilde{f_T}(x^{k+1}) = F_T(x^{k+1},\xi_T) = G_T^{k+1}$
%\item $\nabla \tilde{f_i}(w_{i+1}^k)  = \nabla F_i(w_{i+1}^k,\xi_k) = J_i^{k+1} \quad i \leq T-1$
%\item $\nabla \tilde{f_T}(x^{k+1})  = \nabla F_T(x^{k+1},\xi_T) =  J_T^{k+1}$
%\item $\mathbb{E}[\| J_i^{k+1}\|^2 | \mathscr{F}_k] \leq \sigma_{J_i}^2$
%\end{align*}
%\begin{align}
\end{enumerate}

\end{assumption}
\cref{fi_lips} is a standard smoothness assumption made in the literature on nonlinear optimization. Similarly, Parts 1 and 2 in~\cref{assumption:original_nasa_assumption} are standard unbiasedness and bounded variance assumptions on the stochastic gradient,  common in the literature. At this point, we re-emphasize that the assumptions made in~\cite{zhang2019multi} are stronger than our assumptions above, as they require mean-square smoothness of the individual random functions $G_i$ and their gradients. Parts 3 and 4 are also essential to establish the convergence results in the multi-level case; similar assumptions have been made, for example, in~\cite{yang2019multi-level}. In the next couple of technical results, we provide some properties of composite functions that are required for our subsequent results.
%\begin{align*}
%    \mathbb{E}[\|e_i^{k+1}\|^2 | \mathscr{F}_k] &= \mathbb{E}[\| G_i^{k+1} - f_i(w_{i+1}^k) \|^2 | \mathscr{F}_k] \leq \sigma_i^2=: C_E\tau_k \text{ for some constant } C_E \text{ over } 1 \leq i \leq T-1 \\ \mathbb{E}[\| e_T^{k+1}\|^2 | \mathscr{F}_k] & = \mathbb{E}[\| G_T^{k+1} - f_T(x^k)\|^2 | \mathscr{F}_k] \leq \sigma_T^2=: C_E\tau_k
%\end{align*}



%\subsection*{Main analysis}


\begin{lemma} \label{F_Lipschitz_Constant}
Define $F_i(x) = f_i \circ f_{i+1} \circ \cdots f_T(x)$. Under~\cref{fi_lips}, the gradient of $F_i$ is Lipschitz continuous with constant
\[
L_{\nabla F_i} = \sum_{j=i}^T \left[L_{\nabla f_j} \prod_{l=i}^{j-1} L_{f_l} \prod_{l=j+1}^T L_{f_l}^2\right].
\]

\begin{proof}
We show the result by backward induction. Under~\cref{fi_lips}, gradient of $F_T=f_T$ is Lipschitz continuous and so is that of $F_{T-1}$ since for any $x, y \in X$, we have
\begin{align*}
    \| \nabla F_{T-1}(x) - \nabla F_{T-1}(y)\|  &= \|\nabla f_T(x)\nabla f_{T-1}(f_T(x)) - \nabla f_T(y)\nabla f_{T-1}(f_T(y))\| \\ 
    & \leq \| \nabla f_T(x)\| \| \nabla f_{T-1}(f_T(x)) - \nabla f_{T-1}(f_T(y))\| \\
    &+ \| \nabla f_{T-1}(f_T(y))\| \| \nabla f_T(x) - \nabla f_T(y)\| \\ & \leq (L_{f_T}^2L_{\nabla f_{T-1}} + L_{f_{T-1}}L_{\nabla f_T})\|x -y\|.
\end{align*}
Now, suppose that gradient of $F_{i+1}$ is Lipschitz continuous for any $i \le T-1$. Then, similar to the above relation, $\nabla F_i$ is Lipschitz continuous with constant
\begin{align*}
L_{\nabla F_i} =& L_{F_{i+1}}^2 L_{\nabla f_i} + L_{f_i}L_{\nabla F_{i+1}}\\
= &L_{\nabla f_i} \prod_{j=i+1}^TL_{f_j}^2  + L_{f_i}\sum_{j=i+1}^T \left[L_{\nabla f_j} \prod_{l=i+1}^{j-1} L_{f_l} \prod_{l=j+1}^T L_{f_l}^2\right] \\
=&\sum_{j=i}^T \left[L_{\nabla f_j} \prod_{l=i}^{j-1} L_{f_l} \prod_{l=j+1}^T L_{f_l}^2\right].
\end{align*}
%We prove this by strong induction on $T$. When $T = 2$, we have, $L_{\nabla F} = L_{f_2}^2L_{\nabla f_1} + L_{f_1}L_{\nabla f_2}$. To see this, fix $x, \hat{x} \in X$. We have
%
%\begin{align*}
%    \| \nabla F(x) - \nabla F(\hat{x})\| & = \| \nabla f_1(f_2(x))\nabla f_2(x) - \nabla f_1(f_2(\hat{x}))\nabla f_2(\hat{x})\| \\ & \leq \| \nabla f_2(x)\| \| \nabla f_1(f_2(x)) - \nabla f_1(f_2(\hat{x}))\| + \| \nabla f_1(f_2(\hat{x}))\| \| \nabla f_2(x) - \nabla f_2(\hat{x})\| \\ & \leq (L_{f_2}^2L_{\nabla f_1} + L_{f_1}L_{\nabla f_2})\|x - \hat{x}\|.
%\end{align*}
%
%
%When $T = 3$, we have
%
%\begin{align*}
%    L_{\nabla F} & = (L_{f_2 \circ f_3})^2L_{\nabla f_1} + L_{f_1}L_{\nabla (f_2 \circ f_3)} \\ & = L_{f_2}^2L_{f_3}^2L_{\nabla f_1} + L_{f_1}[L_{f_3}^2L_{\nabla f_2} + L_{f_2}L_{\nabla f_3} ] \\ & = L_{\nabla f_1}L_{f_2}^2L_{f_3}^2 + L_{f_1}L_{\nabla f_2}L_{f_3}^2 + L_{f_1}L_{f_2}L_{\nabla f_3},
%\end{align*}
%
%\noindent where we used base case $T = 2$ and $L_{f_2 \circ f_3} = L_{f_2}L_{f_3}$. By induction hypothesis, when $F_1 = g_1 \circ g_2 \circ \cdots \circ g_{T-1}$, we have
%
%\begin{align*} L_{\nabla F_1} = \sum_{i=1}^{T-1}L_{F_1,i}, \end{align*}
%
%\begin{align*}
%    L_{F_1,i} = \begin{cases} L_{\nabla g_1}\prod_{j=2}^{T-1}L_{g_j}^2 & \text{ if } i = 1 \\ \prod_{j=1}^{i-1}L_{g_j}L_{\nabla g_i}\prod_{j=i+1}^{T-1}L_{g_j}^2 & \text{ if } 1 < i < T-1 \\ \prod_{j=1}^{T-2}L_{g_j}L_{\nabla g_T} & \text{ if } i = T-1 \end{cases} .
%\end{align*}
%
%Suppose $F = f_1 \circ \cdots \circ f_T$. Then by base case and induction hypothesis, we have
%
%\begin{align*}
%    L_{\nabla F} & = L_{f_2 \circ \cdots \circ f_T}^2L_{\nabla f_1} + L_{f_1}L_{\nabla (f_2 \circ \cdots \circ f_T)} \notag \\ & = \prod_{j=2}^TL_{f_j}^2L_{\nabla f_1} + L_{f_1}\sum_{i=2}^{T}L_{f_2 \circ \cdots \circ f_T,i},
%\end{align*}
%
%where
%
%\begin{align*}
%    L_{f_2 \circ \cdots \circ f_T,i} = \begin{cases} L_{\nabla f_2}\prod_{j=3}^{T}L_{f_j}^2 & \text{ if } i = 2 \\ \prod_{j=2}^{i-1}L_{f_j}L_{\nabla f_{i}}\prod_{j=i+1}^{T}L_{f_j}^2 & \text{ if } 2 < i < T \\ \prod_{j=2}^{T-1}L_{f_j}L_{\nabla f_T} & \text{ if } i = T \end{cases} .
%\end{align*}
%
%Combining the previous two equations, we have our conclusion.
\end{proof}
\end{lemma}

We remark that the above result has also been proved in~\cite{zhang2019multi}, Lemma 5.2., with a slightly different proof.



\begin{lemma} \label{new_nasa_grad_F_z_hat_error}
Define $F_i(x) = f_i \circ f_{i+1} \circ \cdots f_T(x)$ and the gradient term $\nabla \bar f_i(x,\bar w_i) = \nabla f_T(x) \nabla f_{T-1}(w_T)\cdots\nabla f_i(w_{i+1})$ with $\bar w_i = (w_{i+1},\ldots, w_T)$ for any $x \in X, w_j \in \bbr^{d_j} \ \  j=i+1,\ldots, T$. Then under~\cref{fi_lips}, we have
%(f_1 \circ \cdots \circ f_T)
\begin{align*}
    \|\nabla F_i(x) - \nabla \bar f_i(x,\bar w_i)\| \leq \sum_{j=i}^{T-1}\frac{L_{\nabla f_j}}{L_{f_j}}L_{f_i} \cdots L_{f_T}\|F_{j+1}(x) - w_{j+1} \|.
\end{align*}
\end{lemma}
\begin{proof}
We show the result by backward induction. The case $i=T$ is trivial. When $i=T-1$, under~\cref{fi_lips}, we have
\begin{align*}
    \| \nabla F_{T-1}(x) - \nabla f_T(x)\nabla f_{T-1}(w_T)\| & = \| \nabla f_T(x) [\nabla f_{T-1}(f_T(x))- \nabla f_{T-1}(w_T)]\| \\
    &\leq L_{\nabla f_{T-1}}L_{f_T}\|f_T(x) - w_T\|.
\end{align*}
Now assume that for any $i \le T-2$,
\begin{align*}
    \|\nabla F_{i+1}(x) - \nabla \bar f_{i+1}(x,\bar w_{i+1} ) \| \leq \sum_{j=i+1}^{T-1}\frac{L_{\nabla f_j}}{L_{f_j}}L_{f_{i+1}} \cdots L_{f_T}\| F_{j+1}(x) - w_{j+1} \|.
\end{align*}
We then have
\begin{align*}
&\|\nabla F_i(x) - \nabla \bar f_i(x,\bar w_i ) \|
    = \|\nabla F_{i+1}(x)\nabla f_i(F_{i+1}(x)) - \nabla \bar f_i(x, \bar w_i )\|\\
&\le \|\nabla f_i(F_{i+1}(x))\| \|\nabla F_{i+1}(x) - \nabla \bar f_{i+1}(x, \bar w_{i+1} )\|\\
&+\|\nabla \bar f_{i+1}(x, \bar w_{i+1})\|\|\nabla f_i(F_{i+1}(x))-\nabla f_i(w_{i+1})\|
\\
&\le L_{f_i} \|\nabla F_{i+1}(x) - \nabla \bar f_{i+1}(x, \bar w_{i+1})\|+L_{\nabla f_i} L_{f_{i+1}} \cdots L_{f_T} \|F_{i+1}(x)-w_{i+1}\|\\
&\le L_{f_i} \sum_{j=i+1}^{T-1}\frac{L_{\nabla f_j}}{L_{f_j}}L_{f_{i+1}} \cdots L_{f_T}\| F_{j+1}(x) - w_{j+1} \|\\
&+L_{\nabla f_i} L_{f_{i+1}} \cdots L_{f_T} \|F_{i+1}(x)-w_{i+1}\|=\sum_{j=i}^{T-1}\frac{L_{\nabla f_j}}{L_{f_j}}L_{f_i} \cdots L_{f_T}\| F_{j+1}(x) - w_{j+1} \|.
\end{align*}
%
%
%Finally, by the chain rule, Lipschitz assumptions, and induction hypothesis,
%\begin{align*}
%    & \| [\nabla (f_1 \circ \cdots \circ f_{T+1})(x) - \nabla f_1(w_2) \cdots \nabla f_T(w_{T+1}) \nabla f_{T+1}(x)]^\top \| \\ & = \| \nabla f_{T+1}(x)^\top[\nabla f_T(f_{T+1}(x))^\top \cdots \nabla f_1(f_2 \circ \cdots \circ f_{T+1}(x))^\top - \nabla f_T(f_{T+1}(x))^\top \nabla f_{T-1}(w_T)^\top \cdots \nabla f_1(w_2)^\top \\ & + \{\nabla f_T(f_{T+1}(x)) - \nabla f_T(w_{T+1})\}^\top \nabla f_{T-1}(w_T)^\top \cdots \nabla f_1(w_2)^\top]  \| \\ & \leq L_{f_{T+1}}\|\nabla f_T(f_{T+1}(x))^\top \cdots \nabla f_1(f_2 \circ \cdots \circ f_{T+1}(x))^\top - \nabla f_T(f_{T+1}(x))^\top \nabla f_{T-1}(w_T)^\top \cdots \nabla f_1(w_2)^\top\| \\ & + L_{f_{T+1}}L_{\nabla f_T}L_{f_{T-1}}\cdots L_{f_1}\|f_{T+1}(x) - w_{T+1}\| \\ & \leq  L_{f_{T+1}}\sum_{j=1}^{T-1}\frac{L_{\nabla f_j}}{L_{f_j}}L_{f_1} \cdots L_{f_T}\| f_{j+1} \circ \cdots \circ f_T \circ f_{T+1}(x) - w_{j+1} \| \\ & + L_{f_{T+1}}L_{\nabla f_T}L_{f_{T-1}}\cdots L_{f_1}\|f_{T+1}(x) - w_{T+1}\|  \\ & = \sum_{j=1}^T \frac{L_{\nabla f_j}}{L_{f_j}}L_{f_1}\cdots L_{f_{T+1}}\|f_{j+1} \circ \cdots \circ f_{T+1}(x) - w_{j+1}\|
%\end{align*}
\end{proof}

\begin{lemma} \label{new_nasa_fjf_T_wj_error}
Under~\cref{fi_lips}, for any $ j \in \{1,\ldots, T-1\}$, we have
\begin{align*}
    \|f_j \circ \cdots \circ f_T(x) - w_j\| & \leq \|f_j(w_{j+1}) - w_j\| + \sum_{\ell = j+1}^T\left(\prod_{i = j}^{\ell - 1}L_{f_i}\right)\|f_{\ell}(w_{\ell+1}) - w_{\ell}\|.
\end{align*}
\end{lemma}
\begin{proof}
%When $T = 3$,
%\begin{align*}
%    \|f_2 \circ f_3(w_4) - w_2\| & \leq  \| f_2 \circ f_3(w_4) - f_2(w_3)\| + \|f_2(w_3) - w_2\| \\ & \leq L_{f_2}\|f_3(w_4) - w_3\| + \|f_2(w_3) - w_2\|
%\end{align*}
We show the results by backward induction. For $j = T-1$, we have
\begin{align*}
    &\|f_{T-1} \circ f_T(w_{T+1}) - w_{T-1} \| \\
    &\leq \| f_{T-1} \circ f_T(w_{T+1}) - f_{T-1}(w_T) \| + \|f_{T-1}(w_T) - w_{T-1}\| \\ & \leq L_{f_{T-1}}\|f_T(w_{T+1}) - w_T\| + \| f_{T-1}(w_T) - w_{T-1}\|.
\end{align*}
Now suppose the result holds for $j+1, j \in \{1,\ldots, T-2\}$. Then, we have
\begin{align*}
  &  \| f_j \circ f_{j+1} \circ \cdots f_T(w_{T+1}) - w_j\| \\
   \leq & \|f_{j} \circ \cdots f_T(w_{T+1}) - f_j(w_{j+1}) + f_j(w_{j+1}) - w_j\| \\
    \leq & L_{f_j}\|f_{j+1} \circ \cdots \circ f_T(w_{T+1}) - w_{j+1}\| + \| f_j(w_{j+1}) - w_j\| \\ 
     \leq & L_{f_j}\left[\| f_{j+1}(w_{j+2}) - w_{j+1}\| + \sum_{\ell = j+2}^T\left(\prod_{i=j+1}^{\ell -1}L_{f_i}\right)\|f_{\ell}(w_{\ell+1}) - w_{\ell}\|\right] \\ & + \|f_j(w_{j+1}) - w_j\| \\  = & \|f_j(w_{j+1}) - w_j\| + \sum_{\ell = j+1}^T\left(\prod_{i=j}^{\ell-1}L_{f_i}\right)\|f_{\ell}(w_{\ell+1}) - w_{\ell}\|,
\end{align*}
where the third inequality follows by the induction hypothesis.
\end{proof}


\begin{lemma} \label{FZ_difference}
Define
\begin{align*}
    R_1 & = L_{\nabla f_1}L_{f_2} \cdots L_{f_T}, \qquad R_j = L_{f_1} \dots L_{f_{j-1}}L_{\nabla f_j}L_{f_{j+1}} \cdots L_{f_T}/L_{f_j}  \quad 2 \le j \leq T-1, \\ 
    C_2  &= R_1, \quad C_j  = \sum_{i=1}^{j-2} R_i \left(\prod_{l=i+1}^{j-1}L_{f_l}\right) \quad 3 \le j \leq T.
    %C_j &=R_1L_{f_2 \circ \cdots \circ f_{j-1}} + R_2L_{f_3 \circ \cdots \circ f_{j-1}} + \cdots + R_{j-2}L_{f_{j-1}} \text{ with } 2 < j \leq T.
\end{align*}
Assume that~\cref{fi_lips} holds. Then for $T \geq 3$,
\beq
    \left\| \nabla F(x) - \nabla f_T(x) \prod_{i=2}^T \nabla f_{T+1-i}(w_{T+2-i}) \right\| \leq  \sum_{j=2}^{T-1} C_j\|f_j(w_{j+1}) - w_j\| + C_T\|f_T(x) - w_T\|
\eeq
\end{lemma}
\begin{proof}
By~\cref{new_nasa_grad_F_z_hat_error} and \cref{new_nasa_fjf_T_wj_error}, we have
\begin{align*}
    &  \left\| \nabla F(x) - \nabla f_T(x) \prod_{i=2}^T \nabla f_{T+1-i}(w_{T+2-i}) \right\| \leq \sum_{j=1}^{T-1}R_j\|f_{j+1} \circ \cdots \circ f_T(x) - w_{j+1}\| \\ & = \sum_{j=1}^{T-2}R_j\|f_{j+1} \circ \cdots \circ f_T(x) - w_{j+1}\| + R_{T-1}\|f_T(x) - w_T\| \\ & = \sum_{j=1}^{T-2}R_j\|f_{j+1}(w_{j+2}) - w_{j+1}\| + \sum_{j=1}^{T-2}R_j\sum_{\ell = j+2}^T\left(\prod_{i=j+1}^{\ell-1}L_{f_i}\right)\|f_{\ell}(w_{\ell +1}) -w_{\ell}\| \\
    &+ R_{T-1}\|f_T(x) - w_T\|.
\end{align*}
{\color{black}
Aggregating the constants for $\|f_j(w_{j+1})-w_j\|$, we get the result.}
%The conclusion follows. To see this, term collecting $\|f_2(w_3)-w_2\|$, we have $C_2$. For $2 < j \leq T$, term collecting $\| f_j(w_{j+1})- w_j \|$, we have $C_j$.}
\end{proof}

\vgap

%\begin{lemma} \label{new_nasa_gradient_error}
%\begin{align*}
%\langle d^k, \nabla F(x^{k+1}) - \hat{z}^{k+1} \rangle \leq \sum_{j=2}^{T-1}C_j \|d^k\|\| f_j(w_{j+1}^k) - w_j^k\| + C_T \|d^k\|\|f_T(x^k) - w_T^k\| + C_T L_{f_T} \tau_k \|d^k\|^2.
%\end{align*}
%\end{lemma}
%\begin{proof}
%This follows from lemma \ref{new_nasa_grad_F_z_hat_upperbound}, Cauchy-Schwarz inequality, and
%\begin{align*}\|f_T(x^{k+1}) - w_T\| \leq L_{f_T}\tau_k\|d^k\| + \|f_T(x^k) - w_T\| \end{align*}
%\end{proof}


%\begin{align*}
%    w_i^{k+1} & = (1-b\tau_k)w_i^k + b\tau_kG_i^{k+1} \tag{0}
%\end{align*}



%In this case, we have

%\begin{align*}
%    A_{k,T} & = f_T(x^{k+1}) - f_T(x^k) \\ A_{k,i} & = f_i(w_{i+1}^{k+1}) - f_i(w_{i+1}^k)
%\end{align*}

%So,
%\begin{align*}
%    \| A_{k,T} \| & \leq L_{f_T}\tau_k \|d^k\|  \\ \| A_{k,i} \| & \leq L_{f_i}\| w_{i+1}^{k+1} - w_{i+1}^k\|
%\end{align*}

%Moreover, in equation $(2),(3),(4),(5)$, set $\hat{e}^{k+1} = 0$ due to $(0)$. In equation for $\|w_i^{k+1} - w_i^k\|$, set $J^{k+1} = 0$ due to $(0)$. \newline

%Define for $1 \leq i < T$,
%\begin{align}
%    A_{k,i} & := f_i(w_{i+1}^{k+1}) - f_i(w_{i+1}^k) \label{original_nasa_A_ki} \\ A_{k,T} & := f_T(x^{k+1}) - f_T(x^k) \label{original_nasa_A_kT}
%\end{align}
%Since $f_i$'s are Lipschitz continuous and using the triangle inequality,
%\begin{align}
%    \| A_{k,T} \| & \leq L_{f_T}\tau_k \|d^k\| \label{original_nasa_A_ki_norm_upperbound}  \\
%    \| A_{k,i} \| & \leq L_{f_i}\| w_{i+1}^{k+1} - w_{i+1}^k\| \label{original_nasa_A_kT_norm_upperbound}
%\end{align}\
\textcolor{black}{The following result also shows the Lipschitz continuity of the gradient of the objective function} of the subproblem \eqnok{def_uk}. One can see \cite{GhaRuswan20} for a simple proof.
\begin{lemma}\label{eta_lips_lemma}
Let $\eta(x,z)$ be defined as
\[
\eta(x,z) = \min_{y \in X}\  \left\{\langle z, y-x \rangle + \frac{\beta}{2} \|y-x\|^2\right\}.
\]
Then the gradient of $\eta$ w.r.t. $(x,z)$ is Lipschitz continuous with the constant \[L_{\nabla \eta} = 2\sqrt{(1+\beta)^2+(1+\tfrac{1}{2\beta})^2}.\]
\end{lemma}

\vgap
\noindent In the next result, we provide a recursion inequality for the error in estimating $f_i(w_{i+1})$ by $w_i$.

\begin{lemma} \label{nasa_lemma_fn_w_error}
Let $\{x^k\}_{k \ge 0}$ and $\{w^k_i\}_{k \ge 0} \ \ 1 \le i \le T$ be generated by~\cref{alg:originalnasa}. Denote
\beq \label{nasa_A_ki}
d^k = u^k - x^k, \qquad w_{T+1}^k \equiv x^k \quad \forall k \ge 0, \qquad A_{k,i} = f_i(w_{i+1}^{k+1}) - f_i(w_{i+1}^k) \quad 1 \le i \le T.
\eeq
\begin{itemize}[leftmargin=0.1in]
\item [a)] For any $i \in \{1,\ldots, T\}$,
\begin{align}
   & \| f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 \leq (1-\tau_k)\| f_i(w_{i+1}^k) - w_i^k\|^2 + \frac{1}{\tau_k}\|A_{k,i}\|^2 + \tau_k^2\|e_i^{k+1}\|^2 
    + r_i^{k+1},\label{nasa_fn_w}\\
   &\|w_i^{k+1} - w_i^k\|^2  \leq \tau_k^2\left[\| f_i(w_{i+1}^k) - w_i^k\|^2 + \|e_i^{k+1}\|^2 - 2\langle e_i^{k+1},f_i(w_{i+1}^k) - w_i^k\rangle \right],\label{nasa_wi_increment_squared}
\end{align}
where
\beq\label{nasa_ri}
    r_i^{k+1} = 2\tau_k \langle e_i^{k+1}, A_{k,i} + (1-\tau_k)(f_i(w_{i+1}^k) - w_i^k) \rangle, \qquad e_i^{k+1}= f_i(w_{i+1}^k)-\bar G_i^{k+1}.
\eeq
\item [b)] If, in addition, $f_i$'s are Lipschitz continuous, we have
\begin{align}
\| f_T(x^{k+1}) - w_T^{k+1}\|^2 &\leq (1-\tau_k)\| f_T(x^k) - w_T^k\|^2 + L_{f_T} \tau_k \|d^k\|^2 + \tau_k^2\|e_T^{k+1}\|^2 + r_T^{k+1}, \\
    \| f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 & \leq (1-\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2 +   \tau_k^2\|e_i^{k+1}\|^2 + \bar{r}_i^{k+1} \notag \\ & 
 + L_{f_i}^2\tau_k \left[\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + \|e_{i+1}^{k+1}\|^2\right]  \qquad   1 \le i \le T-1, \label{nasa_upperbound_fiwi_squared}
\end{align}
where
\begin{align}
    %\bar{r}_{T-1}^{k+1} & = -2\tau_kL_{f_{T-1}}^2\langle e_T^{k+1}, f_T(x^k) - w_T^k\rangle + r_{T-1}^{k+1} \label{original_nasa_rT1_bar} \\
    \bar{r}_{i}^{k+1} & = -2\tau_kL_{f_i}^2\langle e_{i+1}^{k+1},f_{i+1}(w_{i+2}^k)-w_{i+1}^k\rangle + r_i^{k+1}. \label{original_nasa_ri_bar}
\end{align}
\end{itemize}
%\begin{align}
%    \| f_T(x^{k+1}) - w_T^{k+1} \|^2 & \leq (1-b\tau_k)\|f_T(x^k) - w_T^k\|^2 + \frac{1}{b\tau_k}\|A_{k,T}\|^2  + b^2\tau_k^2 \|e_T^{k+1}\|^2 + r_T^{k+1} \label{original_nasa_fn_w_error_T}
%\end{align}
%and
%\begin{align}
%    r_T^{k+1} = 2\tau_k[b\langle e_T^{k+1},A_{k,T}+(1-b\tau_k)(f_T(x^k)-w_T^k)\rangle]. \label{original_nasa_r_T}
%\end{align}
\end{lemma}

\begin{proof}
Noting \cref{def_wi}, \cref{nasa_fn_w}, and \cref{nasa_ri}, we have
\begin{align*}
    \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 & = \|A_{k,i} + f_i(w_{i+1}^k) - (1-\tau_k)w_i^k - \tau_k(f_i(w_{i+1}^k) - e_i^{k+1})\|^2 \\ & = \|A_{k,i} + (1-\tau_k)(f_i(w_{i+1}^k) - w_i^k) + \tau_ke_i^{k+1}\|^2 \\ & = \|A_{k,i} +(1-\tau_k)(f_i(w_{i+1}^k)-w_i^k)\|^2 + \tau_k^2\|e_i^{k+1}\|^2 + r_i^{k+1}.
\end{align*}
%It suffices to show that
%\begin{align*}
%    \|A_{k,i} +(1-b\tau_k)(f_i(w_{i+1}^k)-w_i^k)\|^2 & \leq (1-b\tau_k)\|f_i(w_{i+1}^k)- w_i^k\|^2 + \frac{1}{b\tau_k}\|A_{k,i}\|^2
%\end{align*}
Then, in the view of \cref{nasa_ri}, \cref{nasa_fn_w} follows by noting that
\begin{align*}
   & \|A_{k,i} +(1-\tau_k)(f_i(w_{i+1}^k)-w_i^k)\|^2 \\
    = & \|A_{k,i}\|^2 + (1-\tau_k)^2\|f_i(w_{i+1}^k)-w_i^k\|^2 + 2(1-\tau_k)\langle A_{k,i}, f_i(w_{i+1}^k) - w_i^k\rangle \nonumber\\
     \leq & \|A_{k,i}\|^2 + (1-\tau_k)^2\|f_i(w_{i+1}^k) - w_i^k\|^2 + \left(\frac{1}{\tau_k}-1\right)\|A_{k,i}\|^2 \nonumber\\ & + (1-\tau_k)\tau_k\|f_i(w_{i+1}^k)-w_i^k\|^2 \nonumber\\
    %& = \frac{1}{\tau_k}\|A_{k,i}\|^2 + (1-\tau_k)[(1-\tau_k) + \tau_k]\|f_i(w_{i+1}^k) - w_i^k\|^2 \\
     = & (1-\tau_k)\|f_i(w_{i+1}^k)-w_i^k\|^2 + \frac{1}{\tau_k}\|A_{k,i}\|^2,\label{Ak_fk}
\end{align*}
due to Cauchy-Schwarz and Young's inequalities. Also, \cref{nasa_wi_increment_squared} directly follows from \cref{def_wi} since
\begin{align*}
    \|w_i^{k+1} - w_i^k\|^2 & = \|\tau_k(\bar G_i^{k+1} - w_i^k)\|^2 = \tau_k^2\|f_i(w_{i+1}^k) - w_i^k - e_i^{k+1}\|^2 \\
    & = \tau_k^2\left[\| f_i(w_{i+1}^k) - w_i^k\|^2 + \|e_i^{k+1}\|^2 - 2\langle e_i^{k+1},f_i(w_{i+1}^k) - w_i^k\rangle \right].
\end{align*}
To show part b), note that by \cref{def_xk}, \cref{nasa_A_ki}, and Lipschitz continuity of $f_i$, we have
\[
\| A_{k,T} \| \leq L_{f_T}\| w_{T+1}^{k+1} - w_{T+1}^k\|=L_{f_T} \tau_k \|d^k\|, \qquad \| A_{k,i} \| \leq L_{f_i}\| w_{i+1}^{k+1} - w_{i+1}^k\|,
\]
for $1 \le i \le T-1$. The results then follows by noting \cref{nasa_fn_w} and \cref{nasa_wi_increment_squared}.
\end{proof}

%By definition of $A_{k,T}$ and $G_T^{k+1}$
%\begin{align*}
%    \|f_T(x^{k+1}) - w_T^{k+1}\|^2 & = \|A_{k,T} + f_T(x^k) - (1-b\tau_k)w_T^k - b\tau_k(f_T(x^k) - e_T^{k+1})\|^2 \\ & = \|A_{k,T} + (1-b\tau_k)(f_T(x^k) - w_T^k) + b\tau_ke_T^{k+1}\|^2 \\ & = \|A_{k,T} +(1-b\tau_k)(f_T(x^k)-w_T^k)\|^2 + b^2\tau_k^2\|e_T^{k+1}\|^2 + r_T^{k+1}
%\end{align*}
%It suffices to show that
%\begin{align*}
%    \|A_{k,T} +(1-b\tau_k)(f_T(x^k)-w_T^k)\|^2 & \leq (1-b\tau_k)\|f_T(x^k)- w_T^k\|^2 + \frac{1}{b\tau_k}\|A_{k,T}\|^2
%\end{align*}
%By Cauchy Schwartz and Young's inequality,
%\begin{align*}
%    \|A_{k,T} +(1-b\tau_k)(f_T(x^k)-w_T^k)\|^2 & = \|A_{k,T}\|^2 + (1-b\tau_k)^2\|f_T(x^k)-w_T^k\|^2 + 2(1-b\tau_k)\langle A_{k,T}, f_T(x^k) - w_T^k\rangle \\ & \leq \|A_{k,T}\|^2 + (1-b\tau_k)^2\|f_T(x^k) - w_T^k\|^2 + \frac{(1-b\tau_k)\|A_{k,T}\|^2}{b\tau_k} \\ & + (1-b\tau_k)b\tau_k\|f_T(x^k)-w_T^k\|^2 \\ & = \frac{1}{b\tau_k}\|A_{k,T}\|^2 + (1-b\tau_k)[(1-b\tau_k) + b\tau_k]\|f_T(x^k) - w_T^k\|^2 \\ & = (1-b\tau_k)\|f_T(x^k)-w_T^k\|^2 + \frac{1}{b\tau_k}\|A_{k,T}\|^2
%\end{align*}

We remark that the mini-batch sampling in \eqnok{def_barG} is only used to reduce the upper bound on the expectation of
$\tau_k \|e_{i+1}^{k+1}\|^2$ in the right hand side of \eqnok{nasa_upperbound_fiwi_squared}. Moreover, we do not need this inequality for $i=1$ when establishing the convergence rate of \cref{alg:originalnasa}. Thus, when $T \le 2$, this algorithm converges without using mini-batch of samples in each iteration, as shown in \cite{GhaRuswan20}.
%\begin{lemma} \label{nasa_lemma_increment_w_square}
%Let $\{w^k_i\}_{k \ge 0} \ \ 1 \le i \le T$ be generated by Algorithm~\ref{alg:originalnasa}. Then, we have
%%
%%\begin{align} \| w_T^{k+1} - w_T^k \|^2 \leq \tau_k^2[\textcolor{red}{b^2} \|f_T(x^k) - w_T^k\|^2 + b^2\|e_T^{k+1}\|^2] - 2b^2\tau_k^2 \langle e_T^{k+1}, f_T(x^k) - w_T^k\rangle \label{original_nasa_wT_increment_squared} \end{align}
%%
%%Similarly,
%
%\end{lemma}
%
%\begin{proof}
%%Equation \cref{nasa_wT_increment_squared} and \cref{original_nasa_wi_increment_squared} follow from the following computation:
%
%%\begin{align*}
%%    \|w_T^{k+1}-w_T^k\|^2 & = \|\tau_k(G_T^{k+1} - w_T^k)\|^2 = \tau_k^2\|f_T(x^k) - w_T^k - e_T^{k+1}\|^2 \\
%%    & = \tau_k^2[\|f_T(x^k) - w_T^k\|^2 + \|e_T^{k+1}\|^2 -2\langle e_T^{k+1},f_T(x^k)-w_T^k\rangle]
%%\end{align*}
%\end{proof}
%\begin{lemma} \label{original_nasa_Aki_squared_upperbound}
%For $1 \leq i \leq T-2$,
%\begin{align*}
%    \frac{1}{b\tau_k}\| A_{k,T-1}\|^2 & \leq \textcolor{red}{1}L_{f_{T-1}}^2 \cdot b\tau_k[\| f_T(x^k) - w_T^k\|^2 + \textcolor{red}{1}\|e_T^{k+1}\|^2 - \textcolor{red}{2}\langle e_T^{k+1} , f_T(x^k) - w_T^k \rangle ]
%\end{align*}
%\begin{align*}
%    \frac{1}{b\tau_k}\|A_{k,i}\|^2 & \leq  L_{f_i}^2b\tau_k \|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + L_{f_i}^2b\tau_k\|e_{i+1}^{k+1}\|^2 - 2b\tau_kL_{f_i}^2 \langle e_{i+1}^{k+1}, f_{i+1}(w_{i+2}^k) - w_{i+1}^k \rangle
%\end{align*}
%\end{lemma}
%\begin{proof}
%By lemma \ref{original_nasa_lemma_increment_w_square},
%\begin{align*}
%    \|A_{k,T-1}\|^2 & \leq L_{f_{T-1}}^2\|w_T^{k+1} - w_T^k\|^2 \\ & \leq (L_{f_{T-1}}b\tau_k)^2[\|f_T(x^k) - w_T^k\|^2 + \|e_T^{k+1}\|^2 -2\langle e_T^{k+1},f_T(x^k) - w_T^k\rangle], \\ \|A_{k,i}\|^2 & \leq L_{f_i}^2\|w_{i+1}^{k+1} - w_{i+1}^k\|^2 \\ & \leq (L_{f_i}b\tau_k)^2[\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + \|e_{i+1}^{k+1}\|^2 - 2\langle e_{i+1}^{k+1}, f_{i+1}(w_{i+2}^k) - w_{i+1}^k\rangle]
%\end{align*}
%\end{proof}
%
%\begin{lemma} \label{original_nasa_lemma_upperbound_fiwi_squared}
%\begin{align}
%    \| f_T(x^{k+1}) - w_T^{k+1} \|^2 & \leq (1-b\tau_k) \|f_T(x^k) - w_T^k\|^2 + \frac{L_{f_T}^2 \tau_k \|d^k\|^2}{b} + b^2\tau_k^2 \| e_T^{k+1} \|^2 + r_T^{k+1} \label{original_nasa_upperbound_fTwT_squared}
%\end{align}
%\begin{align}
%    \| f_{T-1}(w_T^{k+1}) - w_{T-1}^{k+1}\|^2 & \leq (1-b\tau_k)\| f_{T-1}(w_T^k) - w_{T-1}^k\|^2 + L_{f_{T-1}}^2b\tau_k \| f_T(x^k) - w_T^k \|^2 \notag \\ & + L_{f_{T-1}}^2b\tau_k \| e_T^{k+1} \|^2 + b^2\tau_k^2 \| e_{T-1}^{k+1}\|^2 + \bar{r}_{T-1}^{k+1} \label{original_nasa_upperbound_fT1wT1_squared}
%\end{align}
%For $i \leq T-2$,
%\begin{align}
%    \| f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 & \leq (1-b\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2 + L_{f_i}^2b\tau_k\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + L_{f_i}^2b\tau_k \|e_{i+1}^{k+1}\|^2 \notag \\ & + b^2\tau_k^2\|e_i^{k+1}\|^2 + \bar{r}_i^{k+1} \label{original_nasa_upperbound_fiwi_squared}
%\end{align}
%where
%\begin{align}
%    \bar{r}_{T-1}^{k+1} & = -2b\tau_kL_{f_{T-1}}^2\langle e_T^{k+1}, f_T(x^k) - w_T^k\rangle + r_{T-1}^{k+1} \label{original_nasa_rT1_bar} \\ \bar{r}_{i}^{k+1} & = -2b\tau_kL_{f_i}^2\langle e_{i+1}^{k+1},f_{i+1}(w_{i+2}^k)-w_{i+1}^k\rangle + r_i^{k+1} \label{original_nasa_ri_bar}
%\end{align}
%\end{lemma}
%\begin{proof}
%By lemma \ref{original_nasa_lemma_fn_w_error} and \ref{original_nasa_Aki_squared_upperbound}, definition of $\bar{r}_{T-1}^{k+1}, \bar{r}_i^{k+1}$, and $\|A_{k,T}\| \leq L_{f_T}\tau_k\|d^k\|$,
%\begin{align*}
%    \|f_T(x^k) - w_T^{k+1}\|^2 & \leq (1-b\tau_k)\|f_T(x^k) - w_T^k\|^2 + \frac{1}{b\tau_k}\|A_{k,T}\|^2 + b^2\tau_k^2\|e_T^{k+1}\|^2 + r_T^{k+1} \\ & \leq (1-b\tau_k)\|f_T(x^k) - w_T^k\|^2 + \frac{L_{f_T}^2\tau_k}{b}\|d^k\|^2 + b^2\tau_k^2\|e_T^{k+1}\|^2 + r_T^{k+1} \\ \|f_{T-1}(w_T^{k+1}) - w_{T-1}^{k+1}\|^2 & \leq (1-b\tau_k)\|f_{T-1}(w_T^k) - w_{T-1}^k\|^2 + \frac{1}{b\tau_k}\|A_{k,T-1}\|^2 + b^2\tau_k^2 \|e_{T-1}^{k+1}\|^2 + r_{T-1}^{k+1} \\ & \leq (1-b\tau_k)\|f_{T-1}(w_T^k) - w_{T-1}^k\|^2 + L_{f_{T-1}}^2b\tau_k\|f_T(x^k) - w_T^k\|^2 + L_{f_{T-1}}^2b\tau_k\|e_T^{k+1}\|^2 \\ & - 2L_{f_{T-1}}^2b\tau_k\langle e_T^{k+1},f_T(x^k) - w_T^k\rangle + b^2\tau_k^2\|e_{T-1}^{k+1}\|^2 + r_{T-1}^{k+1} \\ \|f_i(w_{i+1}^{k+1}) - w_i^{k+1}\|^2 & \leq (1-b\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2 + \frac{1}{b\tau_k}\|A_{k,i}\|^2 + b^2\tau_k^2\|e_i^{k+1}\|^2 + r_i^{k+1} \\ & \leq (1-b\tau_k)\|f_i(w_{i+1}^k) - w_i^k\|^2 + L_{f_i}^2b\tau_k\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + L_{f_i}^2b\tau_k\|e_{i+1}^{k+1}\|^2 \\ & -2b\tau_kL_{f_i}^2\langle e_{i+1}^{k+1},f_{i+1}(w_{i+2}^k) - w_{i+1}^k\rangle + b^2\tau_k^2\|e_i^{k+1}\|^2 + r_i^{k+1}
%\end{align*}
%\end{proof}

\textcolor{black}{Recalling the definition of $F^*$ from Section~\ref{sec:intro} and denoting $w:= (w_1,\dots,w_T)$, we define, for some positive constants $\gamma =(\gamma_1,\ldots, \gamma_T)$, the merit function
\beq\label{merit_function}
    W_\gamma(x,z,w) = F(x) - F^* - \eta(x,z) + \sum_{i=1}^{T-1}\gamma_i \| f_i(w_{i+1}) - w_i\|^2 + \gamma_T \| f_T(x) - w_T\|^2,
\eeq
which will be used in our next result for establishing convergence analysis of \cref{alg:originalnasa}. It is worth noting that  $W_\gamma(x,z,w) \ge 0$ due to that facts that $F(x) \ge F^*, \eta(x,z) \le0$ (by Lemma~\ref{eta_lips_lemma}), and $\gamma >0$. The precise values of the constants $\gamma_1,\ldots, \gamma_T$ will be set later in our analysis. We should also mention that the above summation can start from $i=2$, in which case the convergence analysis is slightly simpler. However, we use~\eqnok{merit_function} in our analysis since, as a byproduct, it gives us an online certificate for the stochastic values of the objective function.} The above function is an extension of the one used in \cite{GhaRuswan20} for the case of $T=2$, to the multi-level setting of $T\ge 1$. A variant of this function (including only the first two terms in \eqnok{merit_function}) was used in the literature as early as \cite{ruszczynski1987linearization} and was used later in \cite{rusz20-1} for nonsmooth single-level stochastic optimization. 
%{\color{red}Another variant of this function in which the square norm is replaced by the norm was also recently used in \cite{rusz20} for case of the nonsmooth functions and general $T \ge 1$.}

%We remark that a simpler variant of this Lyapunov function \eqnok{merit_function} including only the first two terms seems to be . The function \eqnok{merit_function} was used in \cite{GhaRuswan20} for the case of $T=2$. .


\begin{lemma} \label{original_nasa_merit_function_lemma}
Suppose that the sequences $\{x^k,z^k,u^k,w_1^k,\dots,w_T^k\}_{k \geq 0}$ are generated by~\cref{alg:originalnasa} and~\cref{fi_lips} holds.
\begin{itemize}[leftmargin=0.1in]
\item [a)] If
\begin{align}\label{parameter_cond}
&\gamma_1 \ge \lambda >0, \qquad \gamma_j-\gamma_{j-1}L^2_{f_{j-1}}-\lambda >0, \notag\\ %\qquad  \beta \ge \lambda+\gamma_T, \notag\\
&4(\beta-\lambda-\gamma_T)(\gamma_j-\gamma_{j-1}L^2_{f_{j-1}}-\lambda) \ge TC_j^2 \quad j=2,\ldots, T,
\end{align}
where $C_j$'s are defined in~\cref{FZ_difference}, we have
\begin{align}\label{main_recursion}
\lambda \sum_{k=0}^{N-1}\tau_k\left[\|d^k\|^2 + \sum_{i=1}^{T-1}\|f_i(w_{i+1}^k) - w_i^k\|^2 + \|f_T(x^k) - w_T^k\|^2 \right] &\leq W_\gamma(x^0,z^0,w^0)\notag\\
&+\sum_{k=0}^{N-1}R^{k+1},
\end{align}
where
\begin{align}
R^{k+1} &:= \tau_k^2 \sum_{i=1}^{T}\gamma_i \| e_i^{k+1}\|^2+\tau_k \sum_{i=1}^{T-1}\gamma_i L_{f_i}^2 \| e_{i+1}^{k+1}\|^2 + \sum_{i=1}^{T-1}\gamma_i \bar{r_i}^{k+1}+\gamma_T r_T^{k+1} \notag\\
&~~~~~+
\tau_k \langle d^k, \Delta^k\rangle+\frac{(L_{\nabla F}+L_{\nabla \eta})\tau_k^2}{2}\|d^k\|^2 + \frac{L_{\nabla \eta}}{2}\|z^{k+1} - z^k\|^2, \label{def_R_error}\\
 \Delta^k&:= \nabla f_T(x^k) \prod_{i=2}^T \nabla f_{T+1-i}(w^k_{T+2-i})-\prod_{i=1}^T J_{T-i+1}^{k+1},\label{def_deltak}
\end{align}
and $r^{k+1}_i, \bar r^{k+1}_i$ are defined in \cref{nasa_ri} and \cref{original_nasa_ri_bar}, respectively.
\item[b)] If parameters are chosen as
\begin{align}\label{parameter_def}
\gamma_j &:= 2^{j-1}(L_{f_1}\cdots L_{f_{j-1}})^2 \sqrt{T} \quad 2 \leq j \leq T, \qquad \beta \geq \lambda + \gamma_T+\frac{T \max_{2 \leq i \leq T}C_i^2}{4\lambda},\notag\\
\gamma_1 &= \lambda = \frac{1}{2}\min_{2 \leq i \leq T}(\gamma_i - \gamma_{i-1}L_{f_{i-1}}^2)= \frac{\min_{2 \leq i \leq T} \gamma_i}{4}.
\end{align}
Then, conditions in \cref{parameter_cond} are satisfied.
%Suppose
%\begin{align}
%    \bar{\alpha_i}^2 \leq \frac{(\alpha_0 - \lambda)}{T}(\alpha_i - \lambda) \quad \text{ for } 1 \leq i \leq T, \label{original_nasa_merit_function_upperbound_assumption}
%\end{align}
%where
%\begin{align*}
%    \alpha_0 & = \left(a\beta_k - \frac{\gamma_TL_{f_T}^2}{b}\right) \\
%    \alpha_1 & = \gamma_1b, \\ \alpha_i & = b(\gamma_i - \gamma_{i-1}L_{f_{i-1}}^2) \quad \text{ for } 2 \leq i \leq T, \\ \overline{\alpha_1} & := 0 \\
%    \overline{\alpha_i} & = aC_i \quad \text{ for } 2 \leq i \leq T,
%\end{align*}
%and where $C_i$ is defined in lemma \ref{new_nasa_grad_F_z_hat_upperbound}. Note equation \cref{original_nasa_merit_function_upperbound_assumption} is satisfied when we pick
%\begin{align} \lambda = \frac{1}{2}\min_{1 \leq i \leq T}\alpha_i, \label{original_nasa_merit_function_lambda} \end{align}
%and
%\begin{align}
%    \beta_k \geq \frac{1}{a}\left[\frac{T\max_{2 \leq i \leq T}\bar{\alpha_i}^2}{\lambda} + \lambda + \frac{\gamma_TL_{f_T}^2}{b}\right]. \label{original_nasa_merit_function_beta}
%\end{align}
\end{itemize}
%where, for any $k \geq 0$,
%
%\begin{align*}
%    d^k & = u^k - x^k, \\
%    \Delta_k^F & := \left[\prod_{j=1}^{T-1}\nabla f_j(w_{j+1}^k)\right]\nabla f_T(x^{k+1}) - \prod_{i=1}^TJ_i^{k+1} \\
%    \bar{R}^{k+1} & = \bar{r}^{k+1} + a\tau_k^2C_TL_{f_T}\|d^k\|^2
%\end{align*}
%
%and where
%\begin{align*}
%    \bar{r}^{k+1} & = \frac{\tau_k^2}{2}\left[aL_{\nabla F}\|d^k\|^2 + L_{\nabla \eta} \|d^k\|^2 + \sum_{i=1}^T2\gamma_i b^2 \|e_i^{k+1}\|^2\right] \\ & + \sum_{i=1}^{T-1}\gamma_i \bar{r}_i^{k+1} + \gamma_T r_T^{k+1} + \frac{L_{\nabla \eta}}{2}\| z^{k+1} - z^k\|^2 + a\tau_k \langle d^k, \Delta_k^F\rangle + \sum_{j=1}^{T-1}\gamma_j L_{f_j}^2 b\tau_k \|e_{j+1}^{k+1}\|^2
%\end{align*}
\end{lemma}

\begin{proof}
First, note that by~\cref{F_Lipschitz_Constant}, we have
\begin{align}\label{F_lips}
F(x^{k+1}) &\le F(x^k) +\langle \nabla F(x^k), x^{k+1}-x^k \rangle +\frac{L_{\nabla F}}{2}\|x^{k+1}-x^k\|^2 \notag \\
&= F(x^k) +\tau_k \langle \nabla F(x^k), d^k \rangle + \frac{L_{\nabla F}\tau_k^2}{2}\|d^k\|^2.
\end{align}
Second, note that by the optimality condition of \cref{def_uk}, we have
\beq \label{opt_QP}
\langle z^k+\beta(u^k-x^k), x^k-u^k \rangle \ge 0,~\text{which implies}~\langle z^k, d^k \rangle +\beta \|d^k\|^2 \le 0.
\eeq
Then, noting \cref{def_xk}, \cref{def_zk}, and in the view of~\cref{eta_lips_lemma}, we obtain
\begin{align}\label{eta_lips}
&\eta(x^k,z^k)- \eta(x^{k+1},z^{k+1}) \notag\\
&\le \langle z^k+ \beta(u^k-x^k), x^{k+1}-x^k \rangle- \langle u^k-x^k, z^{k+1}-z^k\rangle \notag\\ 
&+\frac{L_{\nabla \eta}}{2} \left[\|x^{k+1}-x^k\|^2 +\|z^{k+1}-z^k\|^2 \right]\notag \\
&= \tau_k \langle 2z^k+ \beta d^k, d^k \rangle- \tau_k \langle d^k, \prod_{i=1}^TJ_{T-i+1}^{k+1}\rangle +\frac{L_{\nabla \eta}}{2} \left[\|x^{k+1}-x^k\|^2 +\|z^{k+1}-z^k\|^2 \right] \notag \\
&\leq -\beta\tau_k \|d^k\|^2 - \tau_k\langle d^k, \prod_{i=1}^TJ_{T-i+1}^{k+1}\rangle
    + \frac{L_{\nabla \eta}}{2}\left[\tau_k^2\|d^k\|^2 + \|z^{k+1} - z^k\|^2 \right].
%& + a\tau_k\left\langle d^k, \left[\prod_{j=1}^{T-1} \nabla f_j(w_j^k)\right]\nabla f_T(x^{k+1}) - \prod_{i=1}^TJ_i^{k+1} \right\rangle \\
\end{align}
Third, noting~\cref{nasa_lemma_fn_w_error}.b), we have
\begin{align}
&\sum_{i=1}^{T-1}\gamma_i \left[\| f_i(w^{k+1}_{i+1}) - w^{k+1}_i\|^2 - \| f_i(w^k_{i+1}) - w^k_i\|^2 \right] \notag\\ 
&\qquad+ \gamma_T \left[\| f_T(x^{k+1}) - w^{k+1}_T\|^2-\| f_T(x^k) - w^k_T\|^2\right]\notag\\
\le& \sum_{i=1}^{T-1}\gamma_i\bigg\{-\tau_k\big[\|f_i(w_{i+1}^k) - w_i^k\|^2- L_{f_i}^2\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 \notag \\
&\qquad - L_{f_i}^2 \| e_{i+1}^{k+1}\|^2 \big]+ \tau_k^2 \|e_i^{k+1}\|^2 + \bar{r_i}^{k+1}\bigg\} \notag\\
&\qquad + \gamma_T \left\{-\tau_k\left[\|f_T(x^k) - w_T^k\|^2 - L_{f_T}^2\|d^k\|^2 \right]+\tau_k^2 \|e_T^{k+1}\|^2 + r_T^{k+1}\right\}\notag\\
=&- \tau_k \bigg\{\gamma_1 \|f_1(w_2^k) - w_1^k\|^2  + \sum_{j=2}^{T-1}[\gamma_j-\gamma_{j-1}L_{f_{j-1}}^2] \|f_j(w_{j+1}^k) - w_j^k\|^2 \notag \\
&\qquad + [\gamma_T-\gamma_{T-1}L_{f_{T-1}}^2]\|f_T(x^k) - w_T^k\|^2\bigg\}+ \sum_{i=1}^{T-1}\gamma_i \bar{r_i}^{k+1}+\gamma_T r_T^{k+1}\notag\\
&\qquad+\tau_k \left[\sum_{i=1}^{T-1}\gamma_i L_{f_i}^2 \| e_{i+1}^{k+1}\|^2+\gamma_T\|d^k\|^2\right]
+\tau_k^2 \sum_{i=1}^{T}\gamma_i \| e_i^{k+1}\|^2.\label{fun_diff}
\end{align}
Combining the above relation with \cref{eta_lips}, \cref{F_lips}, noting definition of merit function in \cref{merit_function}, and in the view of~\cref{FZ_difference}, we obtain
%We compute $W(x^{k+1},z^{k+1},\bar{w}^{k+1}) - W(x^k,z^k,\bar{w}^k)$. Starting with.
%and noting lemma (?), we have
%\begin{align*}
%    \langle d^k, \nabla F(x^{k+1}) - \hat{z}^{k+1}\rangle \leq \sum_{j=2}^{T-1}C_j \|d^k\| \|f_j(w_{j+1}^k) -w_j^k\| + C_T\|d^k\| \|f_T(x^k) - w_T^k\| + C_TL_{f_T}\tau_k \|d^k\|^2
%\end{align*}
%where $\hat{z}^{k+1} = \nabla f_1(w_2^k)\nabla f_2(w_3^k) \dots \nabla f_{T-1}(w_T^k) \nabla f_T(x^{k+1})$.
%Continuing with the computation and using lemma \ref{original_nasa_lemma_upperbound_fiwi_squared},
\begin{align*}
    & W_\gamma(x^{k+1},z^{k+1},w^{k+1}) - W_\gamma(x^k,z^k,w^k)   \\
    &\le -\tau_k(\beta-\gamma_T)\|d^k\|^2+\tau_k \|d^k\|\left[\sum_{j=2}^{T-1} C_j\|f_j(w^k_{j+1}) - w^k_j\| + C_T\|f_T(x) - w_T\|\right]\\
    &\qquad- \tau_k \bigg\{\gamma_1 \|f_1(w_2^k) - w_1^k\|^2  + \sum_{j=2}^{T-1}[\gamma_j-\gamma_{j-1}L_{f_{j-1}}^2] \|f_j(w_{j+1}^k) - w_j^k\|^2 \notag \\
    &\qquad+ [\gamma_T-\gamma_{T-1}L_{f_{T-1}}^2]\|f_T(x^k) - w_T^k\|^2\bigg\}+R^{k+1},\notag
\end{align*}
where $R^{k+1}$ is defined in \cref{def_R_error}. {\color{black}Now, if \cref{parameter_cond} holds, we have
\begin{align*}
    & -\left(\frac{\beta-\gamma_T}{T}\right)\|d^k\|^2- (\gamma_j-\gamma_{j-1}L_{f_{j-1}}^2) \|f_j(w_{j+1}^k) - w_j^k\|^2 + C_j \|d^k\| \|f_j(w^k_{j+1}) - w^k_j\| \\
    &\le -\lambda \Big[\frac{1}{T}\|d^k\|^2 +\|f_j(w_{j+1}^k) - w_j^k\|^2 \Big] \qquad \forall j \in \{1,\ldots,T\},
\end{align*}
which together with the above inequality imply that}
\begin{align}
&W_\gamma(x^{k+1},z^{k+1},w^{k+1}) - W_\gamma(x^k,z^k,w^k) \notag\\
&\le -\lambda \tau_k\left[\|d^k\|^2 + \sum_{i=1}^{T-1}\|f_i(w_{i+1}^k) - w_i^k\|^2 + \|f_T(x^k) - w_T^k\|^2 \right]+R^{k+1}.\notag
\end{align}
Summing up the above inequalities and re-arranging the terms, we obtain \cref{main_recursion}. It can be easily verified that condition \cref{parameter_cond} is satisfied by the choice of parameters in \cref{parameter_def}.
\end{proof}

%\begin{align*}
%    & \leq a\tau_k\langle \nabla F(x^{k+1}), d^k\rangle + \frac{aL_{\nabla F}\tau_k^2}{2}\|d^k\|^2 - a\beta_k \tau_k \|d^k\|^2 \\ & - a\tau_k \left\langle d^k, \left[\prod_{j=1}^{T-1}\nabla f_j(w_{j+1}^k)\right] \nabla f_T(x^{k+1})\right\rangle \\ & + a\tau_k\left\langle d^k, \left[\prod_{j=1}^{T-1}\nabla f_j(w_{j+1}^k)\right]\nabla f_T(x^{k+1}) - \prod_{i=1}^T J_i^{k+1}\right\rangle \\ & + \frac{L_{\nabla \eta}}{2}\left[\tau_k^2\|d^k\|^2 + \|z^{k+1}-z^k\|^2 \right] \\ & + \sum_{i=1}^{T-2}\gamma_i\left[-b\tau_k \|f_i(w_{i+1}^k) - w_i^k\|^2 + L_{f_i}^2b\tau_k\|f_{i+1}(w_{i+2}^k) - w_{i+1}^k\|^2 + L_{f_i}^2b\tau_k \| e_{i+1}^{k+1}\|^2 + b^2\tau_k^2 \|e_i^{k+1}\|^2 + \bar{r_i}^{k+1}\right] \\ & + \gamma_{T-1}[-b\tau_k\| f_{T-1}(w_T^k) - w_{T-1}^k\|^2 + L_{f_{T-1}}^2 b\tau_k \| f_T(x^k) - w_T^k\|^2 + L_{f_{T-1}}^2 b\tau_k \|e_T^{k+1}\|^2 + b^2\tau_k^2 \|e_{T-1}^{k+1}\|^2 + \bar{r}_{T-1}^{k+1}] \\ & + \gamma_T[-b\tau_k\|f_T(x^k) - w_T^k\|^2 + \frac{L_{f_T}^2\tau_k}{b}\|d^k\|^2 + b^2\tau_k^2 \|e_T^{k+1}\|^2 + r_T^{k+1}]
%\end{align*}
%
%By definition of $\bar{r}^{k+1}$, $\Delta_k^F$, and using lemma \ref{new_nasa_gradient_error},
%\begin{align*}
%    & W(x^{k+1},z^{k+1},\bar{w}^{k+1}) - W(x^k,z^k,\bar{w}^k) \\ & \leq -a\beta_k \tau_k \|d^k\|^2 + \frac{\gamma_T L_{f_T}^2 \tau_k}{b}\|d^k\|^2 + a\tau_k \langle d^k, \nabla F(x^{k+1}) - \hat{z}^{k+1} \rangle \\ & + \bar{r}^{k+1} - \gamma_1b\tau_k \|f_1(w_2^k) - w_1^k\|^2  + \sum_{j=2}^{T-1}b\tau_k[\gamma_{j-1}L_{f_{j-1}}^2 - \gamma_j] \|f_j(w_{j+1}^k) - w_j^k\|^2 \\ & + b\tau_k[\gamma_{T-1}L_{f_{T-1}}^2-\gamma_T]\|f_T(x^k) - w_T^k\|^2 \\ & \leq -a\beta_k\tau_k\|d^k\|^2 + \frac{\gamma_TL_{f_T}^2\tau_k}{b}\|d^k\|^2 \\ & + \sum_{j=2}^{T-1}a\tau_kC_j\|d^k\| \|f_j(w_{j+1}^k) - w_j^k\| + a\tau_k C_T\|d^k\| \|f_T(x^k) - w_T^k\| + a\tau_k C_TL_{f_T}\tau_k\|d^k\|^2 \\ & + \bar{r}^{k+1} - \gamma_1 b\tau_k\|f_1(w_2^k) - w_1^k\|^2 + \sum_{j=2}^{T-1}b\tau_k[\gamma_{j-1}L_{f_{j-1}}^2-\gamma_j]\|f_j(w_{j+1}^k) - w_j^k\|^2 \\ & + b\tau_k[\gamma_{T-1}L_{f_{T-1}}^2-\gamma_T]\|f_T(x^k)-w_T^k\|^2 \\ & = -\tau_k\left[\alpha_0\|d^k\|^2 + \sum_{i=1}^{T-1} \alpha_i\|f_i(w_{i+1}^k) - w_i^k\|^2 - \sum_{i=2}^{T-1}\bar{\alpha}_i\|d^k\| \|f_i(w_{i+1}^k) - w_i^k\|\right] + \bar{R}^{k+1} \\ &  -\tau_k[\alpha_T\|f_T(x^k)-w_T^k\|^2 - \bar{\alpha_T}\|d^k\|\| f_T(x^k)-w_T^k\|] \\ & = -\tau_k[\alpha_0\|d^k\|^2 + \sum_{i=1}^{T-1}\alpha_i\|f_i(w_{i+1}^k)-w_i^k\|^2 -\bar{\alpha}_i\|d^k\| \| f_i(w_{i+1}^k) - w_i^k\|] + \bar{R}^{k+1} \\ & -\tau_k[\alpha_T\|f_T(x^k)-w_T^k\|^2 - \bar{\alpha}_T\|d^k\|\|f_T(x^k)-w_T^k\|] \\ & = -\tau_k[\alpha_0\|d^k\|^2 + \sum_{i=1}^{T-1}\alpha_i\|f_i(w_{i+1}^k)-w_i^k\|^2] + \tau_k\sum_{i=1}^{T-1}\bar{\alpha}_i\|d^k\| \| f_i(w_{i+1}^k) - w_i^k\| + \bar{R}^{k+1} \\ & -\tau_k[\alpha_T\|f_T(x^k)-w_T^k\|^2] + \tau_k \bar{\alpha}_T\|d^k\|\|f_T(x^k)-w_T^k\| \\ & = -\tau_k[\alpha_0\|d^k\|^2 + \sum_{i=1}^{T-1}\alpha_i\|f_i(w_{i+1}^k)-w_i^k\|^2] + \tau_k\sum_{i=1}^{T-1}\sqrt{\left(\frac{\alpha_0 - \lambda}{T}\right)(\alpha_i-\lambda)}\|d^k\| \| f_i(w_{i+1}^k) - w_i^k\| + \bar{R}^{k+1} \\ & -\tau_k[\alpha_T\|f_T(x^k)-w_T^k\|^2] + \tau_k \sqrt{\left(\frac{\alpha_0 - \lambda}{T}\right)(\alpha_T-\lambda )}\|d^k\|\|f_T(x^k)-w_T^k\|
%\end{align*}

%where $\bar{R}^{k+1} = \bar{r}^{k+1} + a\tau_k^2C_TL_{f_T}\|d^k\|^2$. \newline

%Put this in $(4)$ and take the expectation \textcolor{red}{Clarification: With respect to $\mathscr{F}_k$, right?}. Write down equation $(3.19)$ and $(3.22)$ in the NASA paper on arxiv for the multi-level case and combine them with equation $(4)$ and $(18)$ in our draft. Now, you need to use a similar argument on the top of page $12$ of the NASA paper. \newline

%Essentially, you get something like

%\begin{align*}
%    & W(x^{k+1},z^{k+1},w^{k+1}) - W(x^k,z^k,w^k) \\ & \leq -\tau_k\left[\sum_{i=1}^T\alpha_0 \|d^k\|^2 + \alpha_i\|f_i(w_{i+1}^k) - w_i^k\|^2 - \bar{\alpha_i}\|d^k\|\| f_i(w_{i+1}^k) - w_i^k\| \right] + \bar{r}^{k+1}
%\end{align*}

%Let $\alpha_0 = \left(a\beta_k - \frac{\gamma_TL_{f_T}^2}{b}\right), \alpha_1 = \gamma_1b, \alpha_i = b(\gamma_i - \gamma_{i-1}L_{f_{i-1}}^2)$, $\overline{\alpha_i} = aC_i$ for $2 \leq i \leq T$, and define $\bar{\alpha}_1 = 0$.

%where the last line follows from equation \cref{original_nasa_merit_function_upperbound_assumption}. The previous equation can be further upper bounded by Young's inquality. Thus,
%\begin{align*}
%    W(x^{k+1},z^{k+1},\bar{w}^{k+1}) - W(x^k,z^k,\bar{w}^k) & \leq -\tau_k\lambda [ \|d^k\|^2 + \sum_{i=1}^{T-1} \|f_i(w_{i+1}^k) - w_i^k\|^2] -\tau_k\lambda \|f_T(x^k)-w_T^k\|^2  + \bar{R}^{k+1}
%\end{align*}
%
%Therefore, for all $N \geq 1$,
%\begin{align*}
%    \lambda \sum_{k=0}^{N-1}\tau_k\left[\|d^k\|^2 + \sum_{i=1}^{T-1}\|f_i(w_{i+1}^k) - w_i^k\|^2 + \|f_T(x^k) - w_T^k\|^2 \right] & \leq W(x^0,z^0,\bar{w}^0) + \sum_{k=0}^{N-1}\bar{R}^{k+1}
%\end{align*}
%
%Finally, we verify equation \cref{original_nasa_merit_function_upperbound_assumption}. \\
%
%Since we require $\alpha_i > 0$ for all $0 \leq i \leq T$, pick $0 < \gamma_T < \frac{ab\beta_k}{L_{f_T}^2}$ and choose $\gamma_i > \gamma_{i-1}L_{f_{i-1}}^2 > 0$ for $2 \leq i \leq T$. Equivalently pick $\frac{\gamma_i}{L_{f_{i-1}}^2} > \gamma_{i-1}$. These inequalities imply
%
%\begin{align*}
%    0 < \gamma_1 < \frac{\gamma_2}{L_{f_1}^2} < \frac{\gamma_3}{L_{f_1}^2L_{f_2}^2} < \frac{\gamma_4}{L_{f_1}^2 \cdots L_{f_3}^2} < \cdots < \frac{\gamma_T}{L_{f_1}^2 \cdots L_{f_{T-1}}^2} < \frac{ab\beta_k}{L_{f_1}^2 \cdots L_{f_T}^2}
%\end{align*}
%
%Pick $\gamma_i$ and $\lambda$ as described in equation \cref{original_nasa_gamma_constants} and \cref{original_nasa_merit_function_lambda}. When $\beta_k$ is chosen as in equation \cref{original_nasa_merit_function_beta}, we have equation \cref{original_nasa_merit_function_upperbound_assumption} holds. To see why, given
%
%\begin{align*}
%    \bar{\alpha}_i^2 \leq \max_{2 \leq i \leq T}\bar{\alpha}_i^2 \leq \frac{(\alpha_0 - \lambda)}{T}\left(\min_{1 \leq i \leq T}\alpha_i-\lambda \right) = \frac{\left(a\beta_k - \frac{\gamma_TL_{f_T}^2}{b}-\lambda\right)}{T}\lambda,
%\end{align*}
%
%Solving for $\beta_k$ yields that equation \cref{original_nasa_merit_function_upperbound_assumption} holds when
%\begin{align*}
%    \beta_k \geq \frac{1}{a}\left[\frac{T\max_{2 \leq i \leq T}\bar{\alpha_i}^2}{\lambda} + \lambda + \frac{\gamma_TL_{f_T}^2}{b}\right]
%\end{align*}

The next technical result helps us to simplify our convergence analysis.

\begin{lemma} \label{Gamma_lemma} Consider a sequence $\{\tau_k\}_{k \geq 0} \in (0,1]$, and define
\begin{align}\label{def_Gamma}
\Gamma_k= \Gamma_1 \prod_{i=1}^{k-1}(1-\tau_i) \qquad k \ge 2, \qquad
\Gamma_1 = \begin{cases}1 & \text{ if } \tau_0 = 1, \\ 1-\tau_0 & \text{otherwise.}\\\end{cases}
\end{align}
\begin{itemize}
\item [a)] For any $k \ge 1$, we have
\[
\alpha_{i,k} = \frac{\tau_i}{\Gamma_{i+1}}\Gamma_k \quad 1 \le i \le k, \qquad \sum_{i=0}^{k-1}\alpha_{i,k}=\begin{cases}1 & \text{ if } \tau_0 = 1, \\ 1-\Gamma_k & \text{otherwise.}\\\end{cases}
\]

\item [b)]Suppose that $q_{k+1} \leq (1-\tau_k)q_k + p_k \ \  k \ge 0$ for sequences $\{q_k,p_k\}_{k \geq 0}$. Then, we have
\[
    q_k \leq \Gamma_k \left[a q_0 + \sum_{i=0}^{k-1}\frac{p_i}{\Gamma_{i+1}}\right], \qquad a = \begin{cases}0 & \text{ if } \tau_0 = 1, \\ 1 & \text{otherwise.}\\\end{cases}
\]
\end{itemize}
\end{lemma}

\begin{proof}
To show part a), note that
\begin{align*}
\sum_{i=0}^{k-1} \alpha_{i,k}&=\Gamma_k \sum_{i=0}^{k-1}\frac{\tau_i}{\Gamma_{i+1}}= \frac{\tau_0 \Gamma_k}{\Gamma_1} + \sum_{i=1}^{k-1}\frac{\tau_i\Gamma_k}{\Gamma_{i+1}} = \frac{\tau_0 \Gamma_k}{\Gamma_1} + \Gamma_k\sum_{i=1}^{k-1}\left(\frac{1}{\Gamma_{i+1}}-\frac{1}{\Gamma_i}\right) \\
&= 1 - \frac{\Gamma_k}{\Gamma_1}(1-\tau_0).
\end{align*}
To show part b), by dividing both sides of the inequality by $\Gamma_{k+1}$ and  noting \cref{def_Gamma}, we have
\[
\frac{q_1}{\Gamma_1} \leq \frac{(1-\tau_0)q_0+p_0}{\Gamma_1},\qquad
\frac{q_{k+1}}{\Gamma_{k+1}} \leq \frac{q_k}{\Gamma_k} + \frac{p_k}{\Gamma_{k+1}} \quad k \ge 1.
\]
Summing up the above inequalities, we get the result.
%Base case: $k = 1$ and by hypothesis,
%\begin{align*}
%q_1 & \leq (1-\alpha_0)q_0 + p_0 \leq \Gamma_1q_0 + \sum_{i=0}^{k-1}\frac{\Gamma_k}{\Gamma_{i+1}}p_i
%\end{align*}
%By induction hypothesis, assume for all $k \geq 1$,
%\begin{align*}
%    q_k & \leq \Gamma_kq_0 + \sum_{i=0}^{k-1}\frac{\Gamma_k}{\Gamma_{i+1}}p_i
%\end{align*}
%For the inductive step, we use induction hypothesis and have
%\begin{align*}
%    q_{k+1} & \leq (1-\alpha_k)q_k + p_k \\ & \leq (1-\alpha_k)\left[\Gamma_kq_0 + \sum_{i=0}^{k-1}\frac{\Gamma_k}{\Gamma_{i+1}}p_i\right] + p_k \\ & = \Gamma_{k+1}q_0 + \sum_{i=0}^{k-1}\frac{\Gamma_{k+1}}{\Gamma_{i+1}}p_i + p_k \\ & = \Gamma_{k+1}q_0 + \sum_{i=0}^k\frac{\Gamma_{k+1}}{\Gamma_{i+1}}p_i
%\end{align*}
%Hence, the conclusion holds for all $k \geq 1$. \newline
\end{proof}

\vgap

The next result shows the boundedness of the error terms in the right hand side of \eqnok{main_recursion} in expectation. This is an essential step in establishing the convergence analysis of the algorithm.


\begin{proposition} \label{original_nasa_big_proposition}
Suppose that~\cref{assumption:original_nasa_assumption} holds and (for simplicity) $\tau_0 = 1$, $ \beta > 0$ for all $k$. Then, for any  $k \geq 1$, we have
\begin{align}
    \beta^2 \mathbb{E}[\|d^k\|^2| \mathscr{F}_{k}] &\leq \mathbb{E}[\|z^k\|^2|\mathscr{F}_{k}] \leq \prod_{i=1}^T\sigma_{J_i}^2, \label{dk_bnd}\\
    %\mathbb{E}[\|z^1-z^0\|^2 | \mathscr{F}_0] & \leq 2\left[\|z^0\|^2 + \prod_{i=1}^T\sigma_{J_i}^2\right] \label{original_nasa_big_proposition_z1z0_error} \\
    \mathbb{E}[\|z^{k+1}-z^k\|^2 | \mathscr{F}_k] & \leq 4\tau_k^2\prod_{i=1}^T\sigma_{J_i}^2. \label{zk_error}
\end{align}
If, in addition, the batch size $b_k$ in~\cref{alg:originalnasa} is set to
\beq\label{def_bk}
b_k = \left\lceil \frac{\max_{1 \le i \le T} L^2_{f_i}}{\tau_k} \right\rceil \qquad k \ge 0,
\eeq
we have
\beq\label{Rk_bnd}
\mathbb{E}[R^{k+1} | \mathscr{F}_k] \leq \tau_k^2 \left[\frac{1}{2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right)\left(\frac{L_{\nabla F}+(1+4\beta^2)L_{\nabla \eta}}{\beta^2} \right) + \sum_{i=1}^T\gamma_i \sigma_{G_i}^2\right]:= \tau_k^2 \sigma^2,
\eeq
where $R^{k+1}$ is defined in \cref{def_R_error}.
%, and
%\begin{align}
%    \sigma^2:= \frac{1}{2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right)\left(\frac{L_{\nabla F}}{\beta^2} + \frac{(1+4\beta^2)L_{\nabla \eta}}{\beta^2} \right) + \sum_{i=1}^T\gamma_i \sigma_{G_i}^2\label{sigma_squared}
%\end{align}
%
%In addition, if $z^0 = 0$, then
%
%\begin{align}
%    \mathbb{E}[\|z^1-z^0\|^2 | \mathscr{F}_0] & \leq 4a^2\tau_0^2 \prod_{i=1}^T\sigma_{J_i}^2 \label{original_nasa_big_proposition_z1z0_error_z0_zero} \\
%    \mathbb{E}[\bar{R}^1|\mathscr{F}_0] & \leq \sigma^2\tau_0^2 \label{original_nasa_big_proposition_error_R1_conditional_expectation}
%\end{align}

\end{proposition}

\begin{proof}
The first inequality in \cref{dk_bnd} directly follows by \cref{opt_QP} and Cauchy-Schwarz inequality. Noting \cref{def_zk}, the fact that $\tau_0 = 1$, and in the view of~\cref{Gamma_lemma}, we obtain
%
%\begin{align*}
%    \Gamma_1:= \begin{cases} 1, & \text{ if } \tau_0 = \frac{1}{a}, \\ 1 -a\tau_0, & \text{ if } \tau_0 < \frac{1}{a}, \end{cases} \quad \Gamma_k:= \Gamma_1 \prod_{i=1}^{k-1}(1-a\tau_i) \quad \text{ for all } k \geq 2,
%\end{align*}
%
%\begin{align*}
%    \frac{z^1}{\Gamma_1} = \frac{(1-a\tau_0)z^0}{\Gamma_1} + \frac{a\tau_0}{\Gamma_1}\prod_{i=1}^TJ_i^1, \quad \frac{z^{k+1}}{\Gamma_{k+1}} = \frac{z^k}{\Gamma_k} + \frac{a\tau_k}{\Gamma_{k+1}}\prod_{i=1}^TJ_i^{k+1} \quad \text{ for all } k \geq 1.
%\end{align*}
%
%Summing up the above inequalities and $\tau_0 = \frac{1}{a}$, we obtain, for any $k \geq 1$,

\begin{align*}
    z^k & = \sum_{i=0}^{k-1}\alpha_{i,k}\left(\prod_{\ell = 1}^T J_{T+1-l}^{i+1}\right)
%, \quad \alpha_{i,k} = \frac{\tau_i}{\Gamma_{i+1}}\Gamma_k, \quad \sum_{i=0}^{k-1}\alpha_{i,k} = 1.
\end{align*}

By convexity of $\| \cdot \|^2$ and conditional independence, we conclude that

\begin{align*}
    \mathbb{E}[\|z^k\|^2 | \mathscr{F}_k] &\leq \sum_{i=0}^{k-1}\alpha_{i,k}\mathbb{E}\left[\left\| \prod_{\ell=1}^TJ_{\ell}^{i+1} \right\|^2 \ \Bigg| \ \mathscr{F}_k\right] & \leq \sum_{i=0}^{k-1}\alpha_{i,k}\prod_{\ell = 1}^T \mathbb{E}[\| J_{\ell}^{i+1}\|^2 | \mathscr{F}_i] \\
    &\leq \sum_{i=0}^{k-1}\alpha_{i,k}\left(\prod_{\ell=1}^T\sigma_{J_{\ell}}^2 \right) = \prod_{\ell =1}^T\sigma_{J_{\ell}}^2.
\end{align*}
%For (b), we have
%
%\begin{align*}
%    \mathbb{E}[\| z^1 - z^0\|^2 | \mathscr{F}_0] & = \mathbb{E}\left[\left\| a\tau_0\left(\prod_{i=1}^TJ_i^1 - z^0\right)\right\|^2 \Bigg| \mathscr{F}_0\right] \leq 2\|z^0\|^2 + 2\mathbb{E}\left[\left\| \prod_{i=1}^TJ_i^1 \right\|^2 \Bigg| \mathscr{F}_0\right] \\ & \leq 2\left[\|z^0\|^2 + \prod_{i=1}^T \sigma_{J_i}^2\right]
%\end{align*}
%
%Similarly and using (a),
Noting \cref{dk_bnd}, we have
\begin{align*}
    \mathbb{E}[\| z^{k+1}-z^k\|^2 | \mathscr{F}_k] & \leq  \tau_k^2 \mathbb{E}\left[\left\| z^k - \prod_{\ell=1}^TJ_{\ell}^{k+1} \right\|^2 \ \Bigg| \ \mathscr{F}_k\right] \\
    &\leq 2\tau_k^2\left\{\mathbb{E}[\|z^k\|^2 | \mathscr{F}_k] + \mathbb{E}\left[\left\| \prod_{\ell=1}^T J_{\ell}^{k+1} \right\|^2 \ \Bigg| \mathscr{F}_k\right]\right\} \\
    & \leq 2\tau_k^2\left(\prod_{\ell=1}^T\sigma_{J_{\ell}}^2 + \prod_{\ell = 1}^T\sigma_{J_{\ell}}^2\right)  = 4\tau_k^2\left(\prod_{\ell=1}^T\sigma_{J_{\ell}}^2\right).
\end{align*}
%By assumption $\mathbb{E}[\| e_i^{k+1} \|^2 | \mathscr{F}_k] \leq C_E\tau_k$ for all $k \geq 0$,
Now, observe that by \cref{nasa_ri}, \cref{original_nasa_ri_bar}, the choice of $b_k$ in \cref{def_bk}, and under~\cref{assumption:original_nasa_assumption}, we have
\begin{align*}
\mathbb{E}[\Delta^k | \mathscr{F}_k] &=0, \qquad \mathbb{E}[e_i^{k+1} | \mathscr{F}_k] =0, \quad \text{implying} \quad \mathbb{E}[r_i^{k+1} | \mathscr{F}_k]=\mathbb{E}[\bar r_i^{k+1} | \mathscr{F}_k]=0,\\
\mathbb{E}[\| e_i^{k+1} \|^2 | \mathscr{F}_k] &=\mathbb{E}[\| \frac{1}{b_k}\sum_{j=1}^{b_k}G_{i,j}^{k+1} - f_i(w_{i+1}^k) \|^2 | \mathscr{F}_k]
\leq \frac{\sigma_{G_i}^2}{b_k}\\
&\qquad \qquad \qquad \qquad \qquad \qquad \qquad  \qquad  \le \min\left\{1, \frac{\tau_k }{\max_{1 \le i \le T} L^2_{f_i}}\right\} \sigma_{G_i}^2.
\end{align*}
Noting \cref{def_R_error}, \cref{dk_bnd}, \cref{zk_error}, and the above observation, we obtain \cref{Rk_bnd}.
%
%
%By variance bound, $(a)$, and $\bar{r_i}^{k+1}$ and $r_T^{k+1}$ have zero conditional mean,
%\begin{align*}
%    \mathbb{E}[\bar{R}^{k+1} | \mathscr{F}_k] & = \mathbb{E}[\bar{r}^{k+1} | \mathscr{F}_k] + a\tau_k^2C_TL_{f_T}\mathbb{E}[\|d^k\|^2 | \mathscr{F}_k] \\ & \leq \mathbb{E}[\bar{r}^{k+1} | \mathscr{F}_k] + \frac{a\tau_k^2C_TL_{f_T}}{\beta_k^2}\left(\prod_{\ell=1}^T\sigma_{J_{\ell}}^2\right) \\ & \leq \frac{\tau_k^2}{2}\left[aL_{\nabla F}\frac{\left(\prod_{i=1}^T\sigma_{J_i}^2\right)}{\beta_k^2} + \frac{L_{\nabla \eta}}{\beta_k^2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right) + \sum_{i=1}^T2\gamma_ib^2C_E\tau_k\right] \\ &  + 2L_{\nabla \eta}a^2\tau_k^2 \left(\prod_{\ell=1}^T \sigma_{J_{\ell}}^2\right) + \sum_{j=1}^{T-1}\gamma_jL_{f_j}^2b\tau_k^2C_E + \frac{a\tau_k^2C_TL_{f_T}}{\beta_k^2}\left(\prod_{\ell=1}^T\sigma_{J_{\ell}}^2\right) \\ & = \tau_k^2\left[\frac{1}{2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right)\left(\frac{aL_{\nabla F}}{\beta_k^2} + \frac{L_{\nabla \eta}}{\beta_k^2} + \frac{2aC_TL_{f_T}}{\beta_k^2} + 4L_{\nabla \eta}a^2\right) + \sum_{i=1}^T\gamma_ib^2C_E\tau_k + \sum_{j=1}^{T-1}\gamma_jL_{f_j}^2bC_E \right] \\ & \leq \tau_k^2\underbrace{\left[\frac{1}{2}\left(\prod_{i=1}^T\sigma_{J_i}^2\right)\left(\frac{aL_{\nabla F}}{\beta_k^2} + \frac{L_{\nabla \eta}}{\beta_k^2} + \frac{2aC_TL_{f_T}}{\beta_k^2} + 4L_{\nabla \eta}a^2\right) + \sum_{i=1}^T\gamma_ib^2C_E + \sum_{j=1}^{T-1}\gamma_jL_{f_j}^2bC_E\right]}_{\sigma^2}
%\end{align*}
%where the last inequality follows from $\tau_k \leq 1$. Finally, when $z^0 = 0$, we have
%\begin{align*}
%    0 & = \|d^0\|^2 \leq \left(\prod_{i=1}^T\sigma_{J_i}^2\right)\beta_k^{-2}.
%\end{align*}
%By $(b)$, we have
%\begin{align*}
%    \mathbb{E}[\|z^1-z^0\|^2 | \mathscr{F}_0] & \leq 2\left[\|z^0\|^2 + \prod_{i=1}^T\sigma_{J_i}^2\right] = 2\prod_{i=1}^T\sigma_{J_i}^2 \leq 4a^2\tau_0^2\prod_{i=1}^T\sigma_{J_i}^2
%\end{align*}
%which implies after computing $\mathbb{E}[R^1|\mathscr{F}_0] \leq \sigma^2\tau_0^2$.
\end{proof}

Observe that \cref{original_nasa_merit_function_lemma} shows that the summation of $\|d^k\|$ and the errors in estimating the inner function values are bounded by summation of error terms $R^k$ which is in the order of $\sum_{k=1}^N \tau_k^2$ as shown in \cref{original_nasa_big_proposition}. This is the main step in establishing the convergence of \cref{alg:originalnasa}. Indeed, $\bar{x} \in X$ is a stationary point of \cref{eq:mainprob}, if $\bar u=\bar{x}$ and $\bar{z}=\nabla F(\bar{x})$, where
\beq\label{def_sub2}
\bar u = \argmin_{y \in X}\  \left\{\langle \bar{z}, y-\bar{x} \rangle + \frac{1}{2} \|y-\bar{x}\|^2\right\}.
\eeq
Thus, for a given pair of $(\bar{x},\bar{z})$, we can define our termination criterion as follows.
\begin{definition}\label{def_Vxz}
A pair of $(\bar{x},\bar{z})$ generated by ~\cref{alg:originalnasa} is called an $\epsilon$-stationary pair, if $\mathbb{E}[\sqrt{V(\bar{x},\bar{z})}] \le \epsilon$, where
\begin{align}
    V(\bar x,\bar z) = \|\bar u-\bar x\|^2 + \|\bar z - \nabla F(\bar x)\|^2, \label{Lyaponuv_function}
\end{align}
and $\bar u$ is the solution to \eqnok{def_sub2}.
\end{definition}
\textcolor{black}{We emphasize that in Definition~\ref{def_Vxz}, we consider a unified termination criterion for both the unconstrained and constrained cases. When $X=\bbr^{d_T}$, $V(\bar x,\bar z)$ provides an upper bound for the $\|\nabla F(\bar x)\|^2$. This can be simply seen from the fact that $\bar u-\bar x = \bar z$ in~\eqref{def_sub2} for unconstrained problems and hence from~\eqref{Lyaponuv_function}, we have
\[
V(\bar x,\bar z) = \|\bar z\|^2+\|\bar z -\nabla F(\bar x)\|^2 \ge \frac 12 \|\nabla F(\bar x)\|^2.
\] 
We also refer the reader to \cite{GhaRuswan20} for the relation between $V(\bar{x},\bar{z})$ and other common gradient-based termination criteria used in the literature such as gradient mapping (\cite{Nest04,Nest07-1,GhaLanZhang16}) and proximal mapping (\cite{DruLew18}). Furthermore, as shown in \cite{GhaRuswan20}, we have
\begin{align}
%\max(1,\beta_k^2)
    V(x^k,z^k) \le \max(1,\beta^2)\|u^k-x^k\|^2 + \|z^k - \nabla F(x^k)\|^2, \label{Lyaponuv_function2}
\end{align}
where $(x^k,u^k, z^k)$ are the solutions generated at iteration $k-1$ of \cref{alg:originalnasa}. Noting this fact, we provide the convergence rate of this algorithm by appropriately choosing $\beta$ and $\tau_k$ in the next results.} 

\begin{theorem}\label{thm:main_theorem_original_nasa}
Suppose that $\{x^k,z^k\}_{k \geq 0}$ are generated by~\cref{alg:originalnasa}, ~\cref{fi_lips} and \cref{assumption:original_nasa_assumption} hold. Also assume that the parameters satisfy \cref{parameter_def} and step sizes $\{\tau_k\}$ are chosen such that
\begin{align}
    \sum_{i=k+1}^N \tau_i\Gamma_i \leq c \Gamma_{k+1} \quad \forall k \geq 0 \text{ and } \forall N \geq 1, c \text{ is a positive constant}. \label{gamma_condition}
\end{align}

\textbf{(a)} For every $N \geq 1$, we have
\beq\label{nasa_main_theorem}
    \sum_{k=1}^N\tau_k \mathbb{E}[\| \nabla F(x^k) - z^k\|^2 | \mathscr{F}_{k}] \leq {\cal B}_1(\sigma^2, N),
\eeq
where
\beq\label{def_B}
{\cal B}_1(\sigma^2,N)=\frac{4cL^2(T-1)}{\lambda}\left[W_\gamma(x^0,z^0,w^0) + \sigma^2 \sum_{k=0}^{N-1} \tau_k^2\right] + c \prod_{\ell=1}^T\sigma_{J_{\ell}}^2 \sum_{k=0}^{N-1} \tau_k^2,
\eeq
$\sigma^2$ is defined in \cref{Rk_bnd} and
\beq\label{def_L}
    L^2 = \max \left\{L_{\nabla F}^2, \max_{2 \leq i \leq T}C_j^2\right\}.
 %   L_j & = 8(T-2)C_j^2 \quad \text{ for all } 2 \leq j < T, \\ L_T & = 8C_T^2, \\ L_0 & = \frac{2L_{\nabla F}^2}{a^2} + 8C_T^2L_{f_T}^2,
\eeq

\textbf{(b)} As a consequence, we have
\begin{align}
    \mathbb{E}[V(x^R,z^R)] &\le  \frac{1}{\sum_{k=1}^{N} \tau_k}\left\{{\cal B}_1(\sigma^2,N)+\frac{\max(1,\beta^2)}{\lambda}\left[W_\gamma(x^0,z^0,w^0)+ \sigma^2 \sum_{k=0}^{N} \tau_k^2\right]\right\},
    \label{nasa_main_theorem2}
%\frac{1}{\sum_{k=0}^{N-1} \tau_k}\left[\frac{[4cL^2(T-1)+\max(1,\beta^2)]}{\lambda}\left[W(x^0,z^0,w^0) + \sigma^2 \sum_{k=0}^{N-1} \tau_k^2\right] + c \prod_{\ell=1}^T\sigma_{J_{\ell}}^2 \sum_{k=0}^{N-1} \tau_k^2\right],
\end{align}
where the expectation is taken with respect to all random sequences generated by the method and an independent random integer number $R \in \{1,\dots, N\}$, whose probability distribution is given by
\begin{align*}
    \mathbb{P}[R = k] = \frac{\tau_k}{\sum_{j=1}^{N}\tau_j}
\end{align*}

\textbf{(c)} If, in addition, the stepsizes are set to

\beq\label{def_tau}
    \tau_0 = 1, \quad \tau_k = \frac{1}{\sqrt{N}} \quad \forall k = 1, \dots, N,
\eeq
we have
\begin{align}
\mathbb{E}[\| \nabla F(x^R) - z^R\|^2 ] &\le  \frac{1}{\sqrt{N}}\left[\frac{4L^2(T-1)\left[W_\gamma(x^0,z^0,w^0) + 2\sigma^2 \right]}{\lambda} +  2\prod_{\ell=1}^T\sigma_{J_{\ell}}^2 \right]\notag\\
&: = \frac{{\cal B}_2(\sigma^2)}{\sqrt{N}},\label{nasa_Fk-zk}\\
\mathbb{E}[V(x^R,z^R)] &\le  \frac{1}{\sqrt{N}}\left[{\cal B}_2(\sigma^2)+\frac{\max(1,\beta^2)}{\lambda}\left[W_\gamma(x^0,z^0,w^0) + 2\sigma^2 \right] \right],\label{nasa_main_theorem3}\\
\mathbb{E}[\| f_i(w_{i+1}^R) - w_i^R \|^2] & \leq  \frac{1}{\lambda\sqrt{N}}\left[W_\gamma(x^0,z^0,w^0) + 2\sigma^2\right] \qquad \qquad i = 1, \dots, T. \label{nasa_main_theorem4}
%\\ \mathbb{E}[\| f_T(x^R) - w_T^R\|^2] & \leq \frac{1}{\lambda\sqrt{N}}\left[W(x^0,z^0,w^0) + 2\sigma^2\right].
\end{align}
\end{theorem}

\vgap

\begin{proof}
We first show part (a). Noting \cref{def_zk}, we have
\[
    \nabla F(x^{k+1}) - z^{k+1} = (1-\tau_k)(\nabla F(x^k) - z^k) + \tau_k (\delta^k+\bar \delta^k +\Delta^k),
\]
where $\Delta^k$ is defined in \cref{def_R_error} and
\[
    \delta^k = \nabla F(x^k) - \nabla f_T(x^k) \prod_{i=2}^T \nabla f_{T+1-i}(w^k_{T+2-i}), \qquad
    \bar \delta^k = \frac{\nabla F(x^{k+1}) - \nabla F(x^k)}{\tau_k}.
\]
Denoting $\bar \Delta_k = \langle \Delta^k, (1-\tau_k)(\nabla F(x^k) - z^k) + \tau_k (\delta^k+\bar \delta^k) \rangle$, we have
\begin{align*}
&\|\nabla F(x^{k+1}) - z^{k+1}\|^2 \\
 =& \|(1-\tau_k)(\nabla F(x^k) - z^k) + \tau_k (\delta^k+\bar \delta^k)\|^2 +\tau_k^2 \|\Delta^k\|^2+2\tau_k \bar \Delta_k \\
\le & (1-\tau_k) \|\nabla F(x^k) - z^k\|^2 + 2\tau_k \left[\|\delta^k\|^2+L_{\nabla F}^2\|d^k\|^2+\bar \Delta_k\right]+\tau_k^2 \|\Delta^k\|^2,
\end{align*}
where the inequality follows from convexity of $\|\cdot\|^2$ and Lipschitz continuity of gradient of $F$. Thus, in the view of~\cref{Gamma_lemma}, we obtain
%
%
%Then, in the view of Lemma~\ref{Gamma_lemma}, we obtain
%\[
%    \nabla F(x^k) - z^k = \sum_{i=0}^{k-1}\alpha_{i,k}[\psi_i + \Delta_i^F] \quad \forall k \geq 1,
%\]
%where
%
%
%Hence,
%
%\begin{align*}
%    \nabla F(x^{k-1}) - z^{k-1} = \sum_{i=0}^{k-2}\alpha_{i,k-1}[\psi_i + \Delta_i^F] = \frac{\Gamma_{k-1}}{\Gamma_k}\sum_{i=0}^{k-2}\alpha_{i,k}[\psi_i + \Delta_i^F] \quad \forall k \geq 2.
%\end{align*}
%
%With these in mind and $\tau_0 = \frac{1}{a}$, for all $k \geq 1$,
%
%\begin{align*}
%    \| \nabla F(x^k) - z^k\|^2 & = \left\| \frac{\Gamma_k}{\Gamma_{k-1}}[\nabla F(x^{k-1}) - z^{k-1}] + \alpha_{k-1,k}[\psi_{k-1} + \Delta_{k-1}^F] \right\|^2 \\ & = \| (1-a\tau_{k-1})[\nabla F(x^{k-1}) - z^{k-1}] + a\tau_{k-1}[\psi_{k-1} + \Delta_{k-1}^F] \|^2 \\ & = \| (1-a\tau_{k-1})[\nabla F(x^{k-1}) - z^{k-1}] + a\tau_{k-1}\psi_{k-1} \|^2 + a^2\tau_{k-1}^2\|\Delta_{k-1}^F\|^2 \\ & + 2a\tau_{k-1}\langle (1-a\tau_{k-1})[\nabla F(x^{k-1}) - z^{k-1}] + a\tau_{k-1}\psi_{k-1}, \Delta_{k-1}^F\rangle \\ & \leq (1-a\tau_{k-1})\| \nabla F(x^{k-1}) - z^{k-1}\|^2 + a\tau_{k-1}\| \psi_{k-1}\|^2 + a^2\tau_{k-1}^2 \|\Delta_{k-1}^F\|^2 \\ & + 2a\tau_{k-1}\langle (1-a\tau_{k-1})[\nabla F(x^{k-1}) - z^{k-1}] + a\tau_{k-1}\psi_{k-1}, \Delta_{k-1}^F\rangle
%\end{align*}
%
%By lemma \ref{new_nasa_recursive_relation_upperbound_1},
\[
    \| \nabla F(x^k) - z^k\|^2 \leq 2\Gamma_k \sum_{i=0}^{k-1}\frac{\tau_i}{\Gamma_{i+1}}\left(\|\delta^i\|^2+L_{\nabla F}\|d^i\|^2+\bar \Delta_i+\frac{\tau_i}{2}\|\Delta^i\|^2\right),
\]
which implies that $ \sum_{k=1}^N \tau_k \|\nabla F(x^k) - z^k\|^2 =$
\begin{align}
    &2\sum_{k=1}^N\tau_k\Gamma_k \sum_{i=0}^{k-1}\frac{\tau_i}{\Gamma_{i+1}}\left(\|\delta^i\|^2+L_{\nabla F}^2\|d^i\|^2+\bar \Delta_i+\frac{\tau_i}{2}\|\Delta^i\|^2\right) \notag\\
    =& 2\sum_{k=0}^{N-1} \frac{\tau_k}{\Gamma_{k+1}}\left(\sum_{i=k+1}^N \tau_i\Gamma_i\right)\left(\|\delta^k\|^2+L_{\nabla F}^2\|d^k\|^2+\bar \Delta_k+\frac{\tau_k}{2}\|\Delta^k\|^2\right)\notag\\
    \le & 2c \sum_{k=0}^{N-1}\tau_k\left(\|\delta^k\|^2+L_{\nabla F}^2\|d^k\|^2+\bar \Delta_k+\frac{\tau_k}{2}\|\Delta^k\|^2\right),
    \label{Fz-zk_error}
\end{align}
where the last inequality follows from~\cref{gamma_condition}.

Now, observe that under~\cref{assumption:original_nasa_assumption}, we have
\[
\mathbb{E}[\bar \Delta_k | \mathscr{F}_k] = 0, \qquad \mathbb{E}[\|\Delta_k\|^2 | \mathscr{F}_k] \le
\mathbb{E}\left[\left\| \prod_{\ell=1}^T J_{\ell}^{k+1} \right\|^2 \ \Bigg| \mathscr{F}_k\right] \le \prod_{\ell=1}^T\sigma_{J_{\ell}}^2.
\]
Moreover, by~\cref{FZ_difference} and the fact that $(\sum_{i=1}^n a_i)^2 \leq n\sum_{i=1}^n a_i^2$ for nonnegative $a_i$'s, we have
\begin{align*}
\|\delta_k\|^2 &=\left\| \nabla F(x) - \nabla f_T(x) \prod_{i=2}^T \nabla f_{T+1-i}(w_{T+2-i}) \right\|^2\\
& \leq  2(T-1) \sum_{j=2}^{T-1} C_j^2\|f_j(w_{j+1}) - w_j\|^2 + 2C_T^2\|f_T(x) - w_T\|^2.
\end{align*}
Combining the above observations with \cref{Fz-zk_error} and in the view of \cref{def_L}, we obtain
\begin{align}
    &\sum_{k=1}^N \tau_k \mathbb{E}[\|\nabla F(x^k) - z^k\|^2 | \mathscr{F}_k ] \le c \prod_{\ell=1}^T\sigma_{J_{\ell}}^2 \sum_{k=0}^{N-1} \tau_k^2  \notag \\
    &+ 4cL(T-1) \sum_{k=0}^{N-1}\tau_k\left( \sum_{j=2}^{T-1} \|f_j(w_{j+1}) - w_j\|^2 + \|f_T(x) - w_T\|^2+\|d^k\|^2\right)\notag
\end{align}
Then, \cref{nasa_main_theorem} follows from the above inequality, \cref{main_recursion}, and \cref{Rk_bnd}.
%where
%\begin{align*}
%    \delta_i := \langle (1-a\tau_i)[\nabla F(x^i) - z^i] + a\tau_i\psi_i,\Delta_i^F \rangle
%\end{align*}
%and observe $\mathbb{E}[\delta_k | \mathscr{F}_k] = 0$. By Young's inequality and Lipschitz assumption,
%
%\begin{align*}
%    \| \psi_i \|^2 & \leq \frac{2L_{\nabla F}^2(1-a\tau_i)^2}{a^2}\|d^i\|^2 + 2\| \nabla F(x^{i+1}) - \hat{z}^{i+1}\|^2
%\end{align*}
%where
%\begin{align*}
%    \hat{z}^{k+1} & = \nabla f_1(w_2^k) \nabla f_2(w_3^k) \cdots \nabla f_{T-1}(w_T^k) \nabla f_T(x^{k+1})
%\end{align*}

%Recall that
%\begin{align*}
%    \| \nabla F(x^{k+1}) - \hat{z}^{k+1}\|  & \leq \sum_{j=2}^{T-1}C_j \| f_j(w_{j+1}^k) - w_j^k\| + C_T\|f_T(x^k) - w_T^k\| + C_TL_{f_T}\|x^{k+1}-x^k\|.
%\end{align*}

%where $C_2:= R_1, C_j := R_1L_{f_2 \circ \cdots \circ f_{j-1}} + R_2L_{f_3 \circ \cdots \circ f_{j-1}} + \cdots + R_{j-2}L_{f_{j-1}} + R_{j-1}$ with $1 < j \leq T$ and where
%\begin{align*}
%    R_1 & = L_{\nabla f_1}L_{f_2} \cdots L_{f_T} \\
%    R_j & = L_{f_1} \dots L_{f_{j-1}}L_{\nabla f_j}L_{f_{j+1}} \cdots L_{f_T} \quad 1 < j \leq T-1
%\end{align*}
%
%By lemma \ref{new_nasa_grad_F_z_hat_upperbound}, using Young's inequality, and using for $x_1, \dots, x_n$ non-negative,
%\begin{align*} \left(\sum_{i=1}^nx_i\right)^2 \leq 2n\sum_{i=1}^nx_i^2,\end{align*}
%
%we have
%\begin{align*}
%    \| \nabla F(x^{i+1}) - \hat{z}^{i+1}\|^2 & \leq 2\left(\sum_{j=2}^{T-1}C_j\|f_j(w_{j+1}^i) - w_j^i\|\right)^2 + 2\left(C_T\|f_T(x^i) - w_T^i\| + C_TL_{f_T}\| x^{i+1} - x^i\|\right)^2 \\ & \leq 2\left(\sum_{j=2}^{T-1}C_j\|f_j(w_{j+1}^i) - w_j^i\|\right)^2 + 4[C_T^2\|f_T(x^i) - w_T^i\|^2 + C_T^2L_{f_T}^2\|x^{i+1} - x^i\|^2] \\ & \leq 2\left[2(T-2)\sum_{j=2}^{T-1}C_j^2\|f_j(w_{j+1}^i) - w_j^i\|^2\right] + 4C_T^2\|f_T(x^i) - w_T^i\|^2 + 4C_T^2L_{f_T}^2\tau_i^2\|d^i\|^2
%\end{align*}
%
%therefore, we can pick
%\begin{align*}
%    L_1 & = 1 \\
%    L_j & = 8(T-2)C_j^2 \quad \text{ for all } 2 \leq j < T, \\ L_T & = 8C_T^2, \\ L_0 & = \frac{2L_{\nabla F}^2}{a^2} + 8C_T^2L_{f_T}^2,
%\end{align*}
%so that
%\begin{align*}
%    \| \psi_i\|^2 \leq L_0\|d^i\|^2 + \sum_{j=2}^{T-1}L_j\|f_j(w_{j+1}^i) - w_j^i\|^2 + L_T\|f_T(x^i) - w_T^i\|^2.
%\end{align*}
%
%Returning to
%\begin{align*}
%    \sum_{k=1}^N\left(\tau_k\Gamma_k\sum_{i=0}^{k-1}\frac{a\tau_i}{\Gamma_{i+1}}\|\psi_i\|^2\right) & \leq \sum_{k=1}^N\left(\tau_k\Gamma_k \sum_{i=0}^{k-1}\frac{a\tau_i}{\Gamma_{i+1}}\left[L_0\|d^i\|^2 + \sum_{j=1}^{T-1}L_j\|f_j(w_{j+1}^i) - w_j^i\|^2 \right. \right. \\ & \left. \left. + L_T\|f_T(x^i)- w_T^i\|^2\right]\right) \\ & = a\sum_{k=0}^{N-1}\left\{\frac{\tau_k}{\Gamma_{k+1}}\left[\sum_{i=k+1}^N\tau_i\Gamma_i\right]\left[L_0\|d^k\|^2 + \sum_{j=1}^{T-1}L_j\|f_j(w_{j+1}^k) - w_j^k\|^2 \right. \right. \\ & \left. \left. + L_T\|f_T(x^k) - w_T^k\|^2\right]\right\} \\ & \leq a\bar{c}\sum_{k=0}^{N-1}\tau_k\left[L_0\|d^k\|^2 + \sum_{j=1}^{T-1}L_j\|f_j(w_{j+1}^k) - w_j^k\|^2 + L_T\|f_T(x^k) - w_T^k\|^2 \right]
%\end{align*}
%
%and
%
%\begin{align*}
%    \sum_{k=1}^N \tau_k\Gamma_k\sum_{i=0}^{k-1}\frac{a^2\tau_i^2}{\Gamma_{i+1}}\|\Delta_i^F\|^2 & = a^2\sum_{k=0}^{N-1}\frac{\tau_k^2}{\Gamma_{k+1}}\left(\sum_{i=k+1}^N \tau_i\Gamma_i\right)\|\Delta_k^F\|^2 \leq \bar{c}a^2\sum_{k=0}^{N-1}\tau_k^2\| \Delta_k^F\|^2
%\end{align*}
%
%where by convexity and oracle assumption, we have
%\begin{align*}
%    \mathbb{E}[\| \Delta_k^F\|^2 | \mathscr{F}_k] \leq 4\left(\prod_{i=1}^T\sigma_{J_i}^2\right)
%\end{align*}
%\end{proof}
%\end{theorem}
%Continuing, we have
%\begin{align*}
%    \sum_{k=1}^N\tau_k\mathbb{E}[\| \nabla F(x^k) - z^k\|^2 | \mathscr{F}_k] & \leq \frac{a\bar{c}}{\lambda}\max_{1 \leq i \leq T}L_i \left[W(x^0,z^0,\bar{w}^0) + \sum_{k=0}^{N-1}\mathbb{E}[\bar{R}^{k+1}|\mathscr{F}_k] \right] \\ & + 4\bar{c}a^2\left(\sum_{k=0}^{N-1}\tau_k^2\right)\prod_{1 \leq i \leq T}\sigma_{J_i}^2 \\ & = \frac{a\bar{c}}{\lambda}\max_{1 \leq i \leq T}L_i\left[W(x^0,z^0,\bar{w}^0) + \sum_{k=0}^{N-1}\sigma^2 \tau_k^2\right] \\ & + 4\bar{c}a^2\sum_{k=0}^{N-1}\tau_k^2 \prod_{1 \leq i \leq T}\sigma_{J_i}^2
%\end{align*}
\vgap
\noindent Part (b) then follows from part (a), \cref{Lyaponuv_function2}, \cref{main_recursion}, and noting that
\[
\mathbb{E}[V(x^R,z^R)] = \frac{\sum_{k=1}^{N}\tau_k V(x^k,z^k)}{\sum_{j=1}^{N}\tau_j}.
\]
%For $(b)$, we have
%\begin{align*}
%    \mathbb{E}[V(x^R,z^R)]  & = \sum_{k=1}^{N-1}\frac{\tau_k}{\sum_{j=1}^{N-1}\tau_j}V(x^k,z^k) \\ & \leq \sum_{k=1}^{N-1}\frac{\tau_k}{\sum_{j=1}^{N-1}\tau_j}\left[\max(1,\beta^2)\|d^k\|^2 + \|z^k-\nabla F(x^k)\|^2\right] \\ & \leq \frac{\max(1,\beta^2)}{\lambda \sum_{j=1}^{N-1}\tau_j}\left[W(x^0,z^0,\bar{w}^0) + \sum_{k=0}^{N-1}\sigma^2\tau_k^2\right] \\ & + \frac{a\bar{c}}{\lambda\sum_{j=1}^{N-1}\tau_j}\max_{1 \leq i \leq T}L_i \left[W(x^0,z^0,\bar{w}^0) + \sum_{k=0}^{N-1}\sigma^2\tau_k^2\right] + \frac{4\bar{c}a^2}{\sum_{j=1}^{N-1}\tau_j}\sum_{k=0}^{N-1}\tau_k^2 \prod_{1 \leq i \leq T}\sigma_{J_i}^2 \\ & = \frac{1}{\sum_{k=1}^{N-1}\tau_k}\{a\bar{c}\left[\frac{1}{\lambda}\left(\max_{1 \leq i \leq T}L_i + \frac{\max(1,\beta^2)}{a\bar{c}}\right)\sigma^2+4a\prod_{1 \leq i \leq T}\sigma_{J_i}^2\right]\left(\sum_{k=0}^{N-1}\tau_k^2\right) \\ & + \frac{1}{\lambda}[a\bar{c}\max_{1 \leq i \leq T}L_i + \max(1,\beta^2)]W(x^0,z^0,\bar{w}^0)\}
%\end{align*}
Part (c) also follows by noting that choice of $\tau_k$ in \cref{def_tau} implies that
\begin{align*}
    \sum_{k=1}^{N} \tau_k \geq \sqrt{N}, \quad \sum_{k=0}^{N} \tau_k^2 = 2, \quad \Gamma_k = \left(1-\frac{1}{\sqrt{N}}\right)^{k-1}, \\ \sum_{i=k+1}^{N}\tau_i\Gamma_i = \left(1- \frac{1}{\sqrt{N}}\right)^k\frac{1}{\sqrt{N}}\sum_{i=0}^{N-k-1}\left(1-\frac{1}{\sqrt{N}}\right)^i \leq \left(1-\frac{1}{\sqrt{N}}\right)^k,
\end{align*}
ensuring condition \cref{gamma_condition} with $c=1$.
%Combining what we have above, we get
%
%\begin{align*} \mathbb{E}[V(x^R,z^R)] & \leq  \frac{1}{\sqrt{N}-1}\{\frac{2}{\lambda}\left(\max_{1 \leq i \leq T}L_i + \max(1,\beta^2)\right)\sigma^2 + 8\left(\prod_{1 \leq i \leq T}\sigma_{J_i}^2\right) \\ & + \frac{1}{\lambda}\left[\max_{1 \leq i \leq T}L_i + \max(1,\beta^2)\right]W(x^0,z^0,\bar{w}^0)\} \end{align*}
%
%and by conclusion of lemma \ref{original_nasa_merit_function_lemma}, we have
%
%\begin{align*}
%    \mathbb{E}[\| f_i(w_{i+1}^R) - w_i^R \|^2] & \leq \frac{1}{\lambda(\sqrt{N}-1)}\left[W(x^0,z^0,\bar{w}^0) + 2\sigma^2\right] \quad \text{ for } i = 1, \dots, T-1  \\ \mathbb{E}[\| f_T(x^R) - w_T^R\|^2] & \leq \frac{1}{\lambda(\sqrt{N}-1)}\left[W(x^0,z^0,\bar{w}^0) + 2\sigma^2\right]
%\end{align*}


\end{proof}
\begin{remark}\label{remark:rmk1}
The result in \eqnok{nasa_main_theorem3} implies that to find an $\epsilon$-stationary point of \eqnok{eq:mainprob} (see,~\cref{def_Vxz}), \cref{alg:originalnasa} requires ${\cal O}(\rho^T T^4/\epsilon^4)$ number of iterations, where $\rho$ is a constant depending on the problem parameters (i.e., Lipschitz constants and noise variances). Thus, the total number of used samples is bounded by
\[
\sum_{k=1}^T b_k = {\cal O}\left(\frac{\rho^T T^6} {\epsilon^6}\right) = {\cal O}_T\left(\frac{1} {\epsilon^6}\right)
\]
due to \eqnok{def_bk} and \eqnok{def_tau}. This bound is much better than $\mathcal{O}_T\left(1/\epsilon^{(7+T)/2}\right)$ obtained in \cite{yang2019multi-level} when $T >4$\footnote{Following the presentation in~\cite{yang2019multi-level}, we only present the $\epsilon$-related $T$ dependence for their result.} . In particular, it exhibits the level-independent behavior as discussed in~\cref{sec:intro}. Note that, we obtain constants of order $\rho^T$, for example, when $\sigma^2_{J_i}$ in~\cref{Rk_bnd} are all equal. We emphasize that~\cite{yang2019multi-level} and~\cite{zhang2019multi} also have such constant factors that depend exponentially on $T$, in their proofs and the final results.
\end{remark}

\begin{remark}\label{remark:rmk1-1}
The bound in \eqnok{nasa_main_theorem4} also implies that the errors in estimating the inner function values decrease at the same rate that we converge to the stationary point of the problem. This is essential to obtain a rate of convergence similar to that of single-level problems. Moreover, \eqnok{nasa_Fk-zk} shows that the stochastic estimate $z^k$ also converges at the same rate to the gradient of the objective function at the stationary point where $x^k$ converges to.
\end{remark}

Although our results for~\cref{alg:originalnasa} show improved convergence rates compared to~\cite{yang2019multi-level}, it is still worse than $\mathcal{O}_T\left(1/\epsilon^4\right)$ obtained in \cite{GhaRuswan20} for the case of $T=2$. Furthermore, the batch sizes $b_k$ is of order $\rho^T$ for some constant $\rho$ which makes it impractical. In the next section, we show that both of these issues could be fixed by a properly modified variant of \cref{alg:originalnasa}.



\iffalse

{\color{blue}
In the discussion, we discuss $\sigma^2 = \mathcal{O}\left(\rho^T\right)$ for some $\rho > 1$.
For $(d)$, Observe that $\max_{1 \leq i \leq T}L_i = \mathcal{O}(T), \lambda = \mathcal{O}(1), \beta_k = \mathcal{O}(2^T)$, so $L_{\nabla \eta} = \mathcal{O}(2^T), W(x^0,z^0,\bar{w}^0) = \mathcal{O}(2^T)$. Therefore, by definition of $\sigma^2$, $\gamma_i$ for $1\leq i \leq T$, and the geometric sum formula, these yield $$\sigma^2 := \rho^T = (fill this up)^T$$

It is easy to see that $\rho > 1$. Using these facts, the conclusion follows.

Hence,
\begin{align}
    \mathbb{E}[V(x^R,z^R)] & = \mathcal{O}\left(\frac{4^T\rho^T}{\sqrt{N}}\right) \label{original_nasa_big_theorem_complexity_lyaponuv} \\ \mathbb{E}[\|f_i(w_{i+1}^R) - w_i^R\|^2] & = \mathcal{O}\left(\frac{\rho^T}{\sqrt{N}}\right) \quad \text{ for } i = 1, \dots, T-1 \label{original_nasa_big_theorem_complexity_fiwi} \\ \mathbb{E}[\|f_T(x^R) - w_T^R\|^2] & = \mathcal{O}\left(\frac{\rho^T}{\sqrt{N}}\right) \label{original_nasa_big_theorem_complexity_fTwT}
\end{align}
}

\fi

